Optimizing Distributed Deployment of Mixture-of-Experts Model Inference in Serverless Computing

With the advancement of serverless computing, running machine learning (ML) inference services over a serverless platform has been advocated, given its labor-free scalability and cost effectiveness. Mixture-of-Experts (MoE) models have been a dominant type of model architectures to enable large models nowadays, with parallel expert networks. Serving large MoE models on serverless computing is potentially beneficial, but has been underexplored due to substantial challenges in handling the skewed expert popularity and scatter-gather communication bottleneck in MoE model execution, for cost-efficient serverless MoE deployment and performance guarantee. We study optimized MoE model deployment and distributed inference serving on a serverless platform, that effectively predict expert selection, pipeline communication with model execution, and minimize the overall billed cost of serving MoE models. Especially, we propose a Bayesian optimization framework with multi-dimensional epsilon-greedy search to learn expert selections and optimal MoE deployment achieving optimal billed cost, including: 1) a Bayesian decision-making method for predicting expert popularity; 2) flexibly pipelined scatter-gather communication; and 3) an optimal model deployment algorithm for distributed MoE serving. Extensive experiments on AWS Lambda show that our designs reduce the billed cost of all MoE layers by at least 75.67% compared to CPU clusters while maintaining satisfactory inference throughput. As compared to LambdaML in serverless computing, our designs achieves 43.41% lower cost with a throughput decrease of at most 18.76%.

==> Sec1-Introduction.tex <==
\section{Introduction}

%what is serverless computing and why is it important to study MoE deployment on this setting
Serverless computing is a cloud computing paradigm that the cloud provider elastically manages the provisioning of resources (servers, functions, containers, storage, etc.) to deploy services according to their user demand \cite{jin2023ditto}. 
%This model abstracts the underlying infrastructure away from developers, allowing them to focus on writing code without worrying about the complexities of server management.  
Serverless computing has been used for serving data analytic applications such as web services %\cwu{tell what exact data analytics applications} 
\cite{jin2023ditto}\cite{zhang2021caerus}. 
In recent years, there has been an increasing trend in adopting serverless computing for machine learning (ML) services, particularly for model inference serving. For example, Gillis \cite{yu2021gillis} studies model partitioning and scheduling for large deep neural network (DNN) inference on AWS
Lambda \cite{Amazon} and Google Cloud Functions \cite{Google}; % and KNIX \cite{Knix}; 
TETRIS \cite{li2022tetris} designs a memory-efficient serverless computing runtime %through tensor sharing 
for DNN inference. 

Deploying ML inference services on a serverless platform is more appealing than using traditional GPU/CPU clusters for several reasons. {\em First}, it frees ML developers from managing hardware resources and virtual machine/container environments, simplifying service deployment and maintenance \cite{mampage2022holistic}. {\em Second}, its pay-as-you-go pricing model ensures cost efficiency by charging only for resources actively used in fine granularity, avoiding unnecessary costs for idle resources \cite{kounev2023serverless}. {\em Third}, %serverless computing offers elastic resource extension, such as 
serverless functions have been provided to support parallelisms needed for large-scale ML model inference like AWS
Lambda Functions %\cwu{AWSLambda is a server but not `functions' - tell what concrete serverless functions on AWSLambda are for ML inference} \
\cite{Amazon}, Google Cloud Functions \cite{Google}, Azure Functions %\cwu{Azure is a cloud platform instead of `functions'} 
\cite{Azure}, and Alibaba Cloud Functions \cite{Alibaba}. State-of-the-art commercial serverless platforms largely support CPU services \cite{Amazon}\cite{Google}\cite{Azure}.
Though GPU-based model inference has been preferred for high serving performance, using CPUs for inference serving has been a viable alternative, given that high-caliber GPUs are often in shortage, CPUs are more available and provide substantial cost savings, while being able to meet application service level objectives (SLOs) \cite{he2024distributed}. 

%what is moe and why is it important
The Mixture-of-Experts (MoE) models have been a dominant type of model architectures to enable large models nowadays \cite{fedus2022switch}, 
achieving high model capacity without increasing computation % The MoE model is a machine learning (ML) architecture designed to enhance model capacity and efficiency by partitioning the problem space among several expert networks 
\cite{du2022glam}\cite{rajbhandari2022deepspeed}. To build a large model using the MoE architecture, layers in a representative DNN model (e.g., Transformer) are replaced by MoE layers. Each MoE layer includes a gating network and multiple parallel expert networks. 
During model inference, each input token to an MoE layer is first evaluated by the gating network, which determines the most relevant expert(s) to handle the token \cite{fedus2022switch}. Then the token is routed to the selected expert(s) for computation, and the processing results are aggregated to produce the MoE layer output. 
MoE models have been widely used to %process complex data and 
serve various tasks, %in a computation-effective manner. For instance, 
e.g., GLaM \cite{du2022glam} %with 1.2 trillion parameters requires half the computation power 
for speech recognition %inference compared to GPT-3 \cite{floridi2020gpt} with 175 billion parameters, 
and SwitchTransformer \cite{fedus2022switch} %achieves a 4$\times$ speedup 
for %text translation and 
text generation. %\cwu{what is being generated}. %over a dense model with the same model quality.
%making MoE models highly valuable for both research and practical applications.

Serving a large MoE model is resource intensive as it requires substantial memory to deploy the parallel experts.
DeepSpeed \cite{rajbhandari2022deepspeed} and Lina \cite{li2023accelerating} adopt expert parallelism to accelerate inference with an expert assigned to a device (mostly GPU) and all-to-all communication to receive inputs from other devices. After deployment, devices incur costs even when idle, making GPU/CPUs more costly than using a serverless platform.
%\cwu{tell why they are resource intensive and more costly than using serverless platform}. However, GPUs are scare and expensive resources, largely needed for model training. % this approach has several drawbacks. First, managing multiple devices incurs labor costs. Second, expensive and scarce devices, especially GPUs, hamper scaling to larger MoE models or handling more inference requests. Third, devices may remain underutilized when few inference requests arrive. 
%CPUs and serverless platforms are potentially beneficial for MoE inference serving. 
%and expert parallelism can still work on serverless platforms by treating a serverless function as a device. Hence, CPU-based serverless computing is suitable for MoE inference serving. 

We advocate serving MoE models in a CPU-based serverless platform, for labor and cost-efficient management %and scaling of resources 
of inference serving. 
Serving large MoE models on serverless computing
has been underexplored. 
%due to substantial challenges in %handling the skewed expert popularity and all-to-all communication bottleneck in MoE model execution, enabling cost-efficient serverless MoE model deployment. 
%Despite its practical importance, there is currently a void in the research on MoE model deployment in serverless computing. This paper addresses this gap by studying the deployment of MoE models in serverless environments. 
The main target for MoE model deployment in a serverless platform is to minimize the billed cost of all MoE layers in serving, for memory usage and execution time of serverless functions that run the MoE layers %refers to the charges on exsiting commercial platforms 
\cite{Amazon}\cite{Google}\cite{Azure}\cite{Alibaba}. 
%The cost is largely proportional to memory usage and computing time of the expert networks \cwu{but it should also be related to non-MoE layers in the whole MoE model}. 
%The memory setup of a serverless function determines its computing speed, as more memory provides more virtual CPUs, enhancing computational power - larger memory usage reduces computing time while smaller memory usage increases computing time. However, 
%Either larger memory usage or higher execution time increases the billed cost of functions. %\cwu{clarify how memory setup can decide computation speed of a serverless function}. 
%Therefore, balance memory usage and computing time of serverless functions is essential to minimize the billed cost in serverless computing. 
%\cwu{not clear how this `Therefore' conclusion is drawn - the previous sentence seems to suggest `minimizing the billed cost requires minimizing memory usage only'}. 
%\cwu{not clear how the above statements leads to the following two challenges:} 
%Two major challenges arise for cost-minimal distributed deployment of MoE model inference in a serverless platform.
%Therefore, reducing memory usage and execution time is essential to minimize the billed cost.
%For memory usage, the memory setup of a serverless function should at least satisfy the minimum required memory for the MoE model part in that function. %, which needs to be obtained in advance as serverless functions are typically deployed with this memory setup before service runs. %For each non-MoE layer and subsequent gating network, this memory can be estimated based on the known parameter size and inference request data size.
%For execution time, the all-to-all operation is the main bottleneck in MoE inference serving \cite{li2023accelerating}. 
Two major challenges arise for cost-minimal distributed deployment of MoE model inference in a serverless platform.


{\em First}, serverless functions are typically deployed with memory size configured before the service runs, and the skewed, %difficult-to-predict 
unknown-beforehand expert selection of input tokens %in the MoE layers 
complicates proactive memory configuration of the functions. In MoE serving, some experts (each run as a serverless function) receive many tokens for processing, % and thus require high memory and computation capacities, 
while others do not. %and this expert popularity is unknown before MoE inference and may vary substantially among different inference tasks (e.g., \cwu{tell the inference tasks whose datasets you used in BO learning}) \cite{li2023accelerating}. 
Intuitively, popular experts should be run on serverless functions with larger memory while non-popular ones use less memory. %The memory is set when a serverless function is deployed before service runs. Hence, the serverless function for each expert should be deployed no later than this expert runs.
Existing MoE serving solutions \cite{he2021fastmoe}\cite{zhai2023smartmoe} in GPU/CPU clusters %employ dynamic resource assignment among experts, 
decide resource assignment for experts %after the expert selection 
during MoE inference, which is infeasible in serverless platforms. Deploying a serverless function takes several minutes. The first time after a serverless function is deployed, it takes a long time for the function to start execution, due to resource initialization %\cwu{tell why it needs a long time} 
(i.e., the cold start issue) \cite{zhang2021caerus}. This would cause long delays in MoE serving if its serverless functions are deployed according to the current demand, degrading efficiency and throughput of inference serving. 
Therefore, the key challenge here is to efficiently and accurately estimate expert popularity before the MoE inference service starts in a serverless platform. This enables optimizing memory configurations for serverless functions, %while satisfying the minimal memory required by experts, 
thereby decreasing the billed cost of MoE serving. %in serverless computing.
%For efficient serverless MoE serving, effective expert selection prediction is necessary to mitigate the impact of skewed expert popularity 
%\cwu{clarify what the impact of skewed expert popularity exactly is}. \cwu{not clear how this challenge is related to cost minimization goal of distributed MoE inference serving}. 


{\em Second}, the scatter-gather communication for token-to-expert routing and expert processing result aggregation at MoE layers is time-consuming, %during inference serving, %and there is currently no improvement for this communication in serverless computing. 
%Data is routed between gating network and multiple experts at each MoE layer, 
%causing bottlenecks 
that may block subsequent operations as non-MoE layers must wait for all experts to complete their computation and communication
\cite{rajbhandari2022deepspeed}. 
%\cwu{add citations}. 
Existing proposals on redesigning MoE scatter-gather communication with pipelining \cite{shi2023pipemoe}\cite{zhang2023mpipemoe} in CPU/GPU clusters are inadequate in serverless platforms. %for several reasons. First, %unlike in CPU/GPU clusters, 
Direct inter-function transfers in a serverless platform are constrained by platform-specified maximum data transfer size (i.e., payload size), while indirect transfers via external storage (e.g., S3 bucket for AWS Lambda \cite{Amazon}) take longer as the data must be saved to external storage and then retrieved. %Second, Pipelining design in serverless platforms is affected by direct and indirect transfer methods: 
Pipelining data transfer with model execution %\cwu{what existing pipelining design are you referring to here? tell what the pipelining does} 
is infeasible with direct transfers: a serverless function retains no data between invocations (i.e., stateless property) and direct data transfers from other functions require re-invocation of the function each time; model parameters that a serverless function uses are not retained during direct transfers and hence need to be reloaded for each re-invocation, resulting in significant time and memory waste. %wasted time and memory for loading parameters without effective computation. 
Indirect transfers between serverless functions rely on external storage, incurring longer communication time and higher cost, adding complexity to pipelining design.
%\cwu{give example} 
%\cwu{but you are also designing some pipelining so need to clarify more why existing proposals are inadequate}, due to their \cwu{what this `their' is referring to?} reliance 
%) and the stateless nature of serverless functions \cwu{clarify why stateless nature of serverless functions makes existing data splitting and pipelining inadequate}. 
%All-to-all communication in serverless functions occupies large execution time, leading to high billed costs. 
This calls for novel communication designs tailored to MoE inference in serverless platforms.
%All-to-all communication is involved in the execution of serverless functions, and increases execution time,\cwu{Clarify how all-to-all communication impacts the billed cost by affecting memory utilization and computational efficiency} therefore leading to a larger billed cost, highlighting the need for novel designs tailored to MoE inference in a serverless platform. 

%describe the solution and provide high level intuition on why it works
Tackling these challenges, we design a serverless MoE inference solution that effectively predicts
expert popularity, pipelines MoE communication with model
execution, and optimally deploys MoE model for distributed inference, that minimize the billed cost of all MoE layers in MoE model serving. %of all MoE layers, 
We propose a Bayesian optimization (BO) framework with multiple ${\bf \epsilon}$-greedy search (GS) to learn expert popularity and optimize MoE
deployment for billed cost minimization. %where iterative trials are conducted to achieve the optimal billed cost for all MoE layers by executing our designed serverless MoE inference solution. 
%In the first adjustment period, the framework collects real billed costs using a real-world dataset, and in the following periods, it adjusts predictions based on the real inference requests encountered after the last adjustment. 
%\cwu{clarify what feedback}
%After completing fine-tuning, the framework keeps inactive when our fine-tuned serverless MoE inference solution to execute for real inference request.
%We propose a offline Bayesian optimization (BO) framework with multiple ${\bf e}$-greedy search (GS) to fine-tune expert selection prediction by iteratively predicting expert selection, executing pipelined all-to-all communication and distributed model deployment, and collecting real billed cost of all MoE layers.feedback 
%The Bayesian decision-making predictor uses adjusted maximum posterior probability given token features to predict a new token's expert selection. The policy maker consists of Mixed-Integer Quadratically Constrained Programming (MIQCP) solvers and an Optimal Deployment Selection (ODS) algorithm, which decides how to improve all-to-all communication (e.g., scatter and pipeline operations), set the memory size of serverless functions, and replicate these functions.
Our main %techniques and 
contributions are summarized as follows:

%summarize the contribution
%$\triangleright$ We propose a Bayesian decision-making approach for expert selection prediction, using the maximum posterior given the designed token features \cwu{this appears to be standard Bayesian approach and what the novelty/contribution is? careful feature design or what?}. \cwu{no need to list all designed features but tell `contribution' in this design:}The token features consist of the token ID, position ID, and attention ID (i.e., the ID of the token with the highest relevance to the token under consideration), and the posterior is derived from new data and profiled data distributions \cwu{what's new here?}. 
%\cwu{rewrite the following sentence to tell what the `contribution' is - finetuning what for better prediction:} We form a key-value dataset table to save profiled data, which can be fine-tuned using runtime feedback from model inference \cwu{not clear why and how a table can be fine-tuned}.

$\triangleright$ We design a novel Bayesian decision-making approach for expert selection prediction, including a comprehensive token feature design, a novel posterior calculation approach, and an adjustable key-value dataset table. We analyze the MoE inference process to extract relevant token features. The posterior calculation incorporates real request distributions to refine the posterior using profiled data. The key-value dataset table is adjusted %by changing existing values and adding 
with new key-value pairs according to feedback from model inference, which are used to update the profiled data probabilities and improve prediction accuracy.

$\triangleright$ We propose several scatter-gather communication designs for a serverless platform%by changing data transfer as
: indirect transfers with flexible pipeline operations %\cwu{change this term `scatter and pipeline operations' - not using scatter in the term} 
via external storage,  simple indirect transmissions without pipelining, %\cwu{not clear what simple indirect transmission does}, 
and simple direct invocation of serverless functions without pipelining. As different designs perform the best in terms of execution time under different scenarios, %inference request batch sizes, 
selecting a proper scatter-gather communication design affects billed cost saving in serverless MoE inference. %\cwu{not clear why `direct invocation of serverless functions' is an all-to-all communication method}. \cwu{%tell which all-to-all method to use in what situation, and 
%how they help with the untimate goal of cost saving in serverless MoE inference.}
%We formulate the problem of distributed deployment for MoE model inference to minimize the billed cost across all layers.

$\triangleright$ We formulate optimal deployment of distributed MoE inference on a serverless platform into a mixed-integer quadratically constrained programming (MIQCP) problem, which chooses one of the proposed scatter-gather communication designs,
sets memory configurations of expert serverless functions,
and determines the number of function replicas. %that includes Mixed-Integer Quadratically Constrained Programming (MIQCP) solvers and 
We design an optimal deployment selection (ODS) algorithm, achieving a billed cost of all MoE layers upper bounded by a constant ratio of the optimal solutions. %\cwu{give the highlight/contribution of this algorithm design, any performance guarantee} % and whether the algorithm is running periodically to redeploy the MoE model.

%$\triangleright$ We propose a offline BO framework with multiple ${\bf e}$-GS to optimize overall operation of the serverless MoE inference system. The BO framework iteratively fine-tunes the key-value dataset table for expert selection prediction using the real billed cost of all MoE layers%\cwu{what feedback} feedback 
%from previous optimal MoE deployment, %by the policy maker. 
%and then \cwu{compute optimal MoE deployment based on new expert selection prediction again?}. 
%The multiple \({\bf e}\)-GS balances exploration and exploitation when finding the different key-value pairs in the dataset table \cwu{not clear how it is related to expert selection prediction and the BO framework}.

$\triangleright$ We propose a BO framework with multiple ${\bf \epsilon}$-GS to optimize %overall operation of the serverless MoE inference system
expert selection predictions and distributed deployment of the MoE model. The BO framework iteratively adjusts the key-value dataset table for expert selection prediction using %the real 
feedback billed cost of all MoE layers in serving. %In the first period to adjust, the framework collects real billed costs on a real-world dataset, and in the following periods, it adjusts predictions based on the real inference requests encountered after the last adjustment. Each adjustment involves iteratively predicting expert selections to optimally deploy MoE model, thereby identifying high-performing key-value pairs that minimize the billed cost of all MoE layers.After each adjustment, the framework becomes inactive and the adjusted expert selection prediction works on optimal MoE deployment for real inference requests. 
The expert predictions then serve as input for optimal MoE model deployment, which further provides cost feedback for dataset table update. The multiple ${\bf \epsilon}$-GS balances exploration of different key-value pairs in the dataset table and exploitation of %currently known
high-performing key-value pairs, in dataset table update. % to minimize the billed cost of all MoE layers.

 
$\triangleright$ We implement our designs on AWS Lambda using Pytorch and Optuna packages. %\cwu{give some system implementation highlights, e.g., what platform/library used}. %system to minimize the billed cost of all MoE layers of a MoE model distributed in serverless computing for inference, consisting of an expert selection predictor, an policy maker and a feedback processer.
Extensive experiments %on AWS Lambda 
show that our designs reduce the billed cost of all MoE layers by at least 75.67$\%$ compared to inference over CPU clusters, while maintaining a satisfactory inference throughput. %significantly exceeding human reading levels, and 
%\cwu{revise the following according to my comments in abstract} 
by at least 43.41$\%$ compared to LambdaML \cite{lambdaml} in serverless computing, with a throughput decrease of at most 18.76$\%$. 


\iffalse
\section{Introduction}%not modified yet
Serverless computing has emerged as an alternative to traditional hardware-cluster-based approaches for distributed machine learning (ML) inference \cite{liu2022funcpipe}, due to several appealing benefits. {\em First}, serverless computing can free ML developers from the management hassle of hardware clusters and virtual machine (VM) environments \cite{mampage2022holistic}. {\em Second}, the pay-as-you-go pricing plan \cite{kounev2023serverless} of serverless computing ensures cost efficiency by charging only for actively utilized resources, avoiding unnecessary bills for idle resources. {\em Next}, serverless computing provides an elastic extension of resources, such as serverless functions \cite{herbst2013elasticity}.
%\cite{klimovic2018pocket}. 
This elastic extension facilitates parallelism in ML model inference, beneficial for large-scale ML model inference. 

%As a large-scale ML model, 

The Mixture-of-Experts (MoE) architecture has been adopted to enlarge capacity of deep neural network (DNN) models,  by adopting parallel model structures (termed {\em experts}) without increasing extra computation \cite{du2022glam}\cite{rajbhandari2022deepspeed}. Different from traditional dense DNNs that involve all parameters in the inference, the parallel expert structure (termed {\em MoE layers}) sparsely activates experts. In MoE model inference, inputs (e.g., tokens) are routed to different experts for processing. These experts are dynamically selected by a lightweight trainable gating network according to implicit routing rules. The routing rules mainly refer to token-based routing \cite{lewis2021base}, task-based routing \cite{kudugunta2021beyond}, and expert choice routing \cite{zhou2022mixture}. Here we focus on the token-based routing rule, which routes a token to the top-$k$ ($k\geq 1$) best experts based on implicit features of this token. To improve resource utilization in MoE model inference in traditional GPU clusters, a number of studies exist, e.g., %expert parallelism is commonly adopted
to assign experts on different computing devices \cite{lepikhin2020gshard} and to adopt data parallelism on non-MoE layers to process batch data simultaneously \cite{chen2022ta}. However, unavoidable resource idling (e.g. idle MoE layers when inferencing in non-MoE layers) exists, adding to the resource cost in traditional clusters. %still require to be billed once rented. 
This motivates our study on distributing MoE inference in elastically pay-as-you-go serverless computing platforms, for cost reduction with serving performance guarantees. 

Two major challenges exit on optimizing distributed deployment of MoE model inference in a serverless computing platform. 
{\em First}, the expert popularity at the MoE layers is skewed and unknown beforehand, which prevents proactive memory setup of the serverless functions for MoE layers. Some experts bear high workloads while some experts are idle at the same MoE layer. % due to the sparse activations. The skewed expert popularity can significantly lower resource utilization and increase execution time.  To mitigate this issue, 
Some works \cite{he2021fastmoe}\cite{zhai2023smartmoe} on MoE inference in traditional GPU clusters apply dynamic resource assignment at MoE layers. However, such dynamic assignment is not feasible in a serverless computing platform due to its slow cold start problem \cite{zhang2021caerus}, %leading to the 
requiring distributed deployment before each request's inference starts. Distributed deployment in advance in serverless computing requires expert selection prediction to mitigate impact of the %unknown
skewed expert popularity. {\em Second}, the all-to-all communication around the MoE layers is time consuming during inference. Assuming data parallelism is applied to non-MoE layers (including the gating network), a MoE layer is required to receive tokens routed by several gating networks and to send the outputs to the following non-MoE layers, in which the split shapes or dimensions are different in two scatter operations before and after data exchange. This causes a bottleneck blocking subsequent operations in MoE model inference. To alleviate this problem, existing studies \cite{singh2023hybrid}\cite{shi2023pipemoe}\cite{zhang2023mpipemoe} %in traditional hardware clusters 
redesign the all-to-all communication by splitting the transferred data along different dimensions and pipelining the transfers. However, different from traditional GPU clusters, external storage is relied on for large data exchange in a serverless computing platform, as the serverless functions retain no data between invocations - called the stateless property \cite{kounev2023serverless}. This calls for a different all-to-all communication design.



An expert selection prediction method is proposed based on a Bayesian inference framework, given designed token features (token ID, position ID and attention ID, i.e., ID of the token with the highest relevance to the token under consideration). We propose an all-to-all communication design on the serverless computing platform, by flexibly applying pipeline operations with some hyper-parameters (e.g. pipeline degree). This pipeline degree decides whether a split batch of data requires external storage for its transfer between MoE and non-MoE layers, or not. We formulate a distributed deployment problem of MoE model inference in serverless computing, that minimizes the billed cost of all MoE layers by jointly selecting the memory type of serverless functions and setting the hyper-parameters of all-to-all communication. 
Based on these designs, we propose a Bayesian optimization (BO) algorithm %at an overall level
that minimizes the billed cost of all MoE layers by iteratively finetuning the expert selection prediction upon new dataset tables and optimizing distributed deployment based on our designed all-to-all communication. In summary, we make the following contributions:

%\begin{itemize}
    %\item 
$\triangleright$ We propose an expert selection prediction method with a Bayesian inference framework, given the designed token features. The prediction can be finetuned upon each new dataset table from runtime feedback of model inference on new data.

$\triangleright$ We propose an all-to-all communication design in the serverless computing platform to flexibly apply pipeline operations on transferred data, coping with indirect transmission through external storage and direct invocation of serverless functions.

$\triangleright$ We formulate the distributed deployment problem of MoE model inference to minimize the billed cost of all MoE layers.
We propose a BO algorithm 
that iteratively finetunes the expert selection prediction and optimizes the distributed deployment.
%\end{itemize}

$\triangleright$ We implement a system to optimize distributed deployment of MoE model inference in serverless computing, consisting of an expert selection predictor, an MIQCP solver and a BO solver. The experiments show that our design reduces the billed cost of all MoE layers by at least xxx$\%$ compared to inference over CPU clusters and by at least xxx$\%$ compared to over-provisioning in serverless computing.
\fi
%\cwu{system implementation and experimental results are usually summarized as a contribution point.}

==> Sec2-Related_Work.tex <==
\section{Background and Motivation}
\subsection{Serverless Computing}\label{secIIA}

\begin{figure}[htbp]
\centerline{\includegraphics[width=0.5\textwidth]{figs/Visio-serverless computing.pdf}}
\vspace{-3mm}
\caption{Overview of MoE model deployment on a serverless platform.}% \cwu{the figure can be more detailed, e.g., with multiple serverless functions shown to deploy parts of the MoE model - learn from how other serverless computing system papers draw such figures}}
\label{ServerlessComputing}
\vspace{-4mm}
\end{figure}

Serverless computing is a cloud computing paradigm that provides Functions as a Service (FaaS). A serverless function is a piece of code running %virtually 
in a cloud infrastructure for applications or services, without the need of the developer to provision or manage the resources. These functions can be triggered by various events \cite{kounev2023serverless}, such as inference requests. 
Serverless functions are stateless, that they retain no data from their previous execution. %\cwu{no data at all? then what are the data transferred for invocation between serverless functions?} 
Serverless functions obtain data inputs mainly in two ways: from output %\cwu{output} 
of other functions or from an external storage %(e.g., Amazon S3 bucket \cite{s3} for Amazon Lambda \cite{Amazon}). 
A function can directly transfer output to another function as input when invoking the latter, and a {\em payload} size limits the maximal
data transfer size between functions.  
When the data exceeds the payload size, external storage is used for relaying data between two functions \cite{jin2023ditto}\cite{yu2021gillis}. 
External storage can also store other data needed by serverless functions, such as %other input/output data and
model parameters.

Serverless functions, along with external storage, Docker image manager (e.g., ECR \cite{ecr} for Amazon Lambda \cite{Amazon}), and serverless function deployment manager (e.g., step function \cite{step_func} on Amazon Lambda \cite{Amazon}) %, Google Cloud Workflows \cite{Google_cloud_workflows})
can be used for ML inference. 
% As shown in Fig.~\ref{ServerlessComputing}, inference serving of an MoE model can be performed on a serverless platform by splitting the MoE model, building a Docker image for each split model layer, \cwu{images for model layers?}, 
% pushing images to Docker image manager, \cwu{to where}, 
% saving model parameters in external storage, %{in where}, 
% creating a serverless function for each Docker image, \cwu{each running what - model layers?}, 
% and deploying them using a serverless function manager.
As shown in Fig.~\ref{ServerlessComputing}, deployment of an MoE model for inference serving on a serverless platform involves several steps. First, the MoE model is partitioned: the MoE layer adopts expert parallelism, while the non-MoE layers are grouped and distributed according to model parallelism. %each expert is separated individually, each non-MoE layer is grouped with the subsequent gating network, and the final non-MoE layer is isolated separately. 
Next, each model partition is built as a Docker image, which is then pushed to the Docker image manager, with its model parameters stored in external storage. Finally, each Docker image is assigned to a serverless function and these functions are deployed into the serverless platform by a serverless function manager. After deployment, inference requests from service users are stored in external storage and retrieved by the deployed MoE model for inference serving. During inference, each serverless function loads its model parameters and intermediate computation results from external storage, and saves intermediate results back to external storage. %Output data is also stored in external storage for users to access.
%\cwu{Fig.~\ref{ServerlessComputing} needs to be made clearer (all icons in the figure need to be defined otherwise readers may not get what it is), as well as the steps described here, e.g., mention docker, expert and non-MoE layer}.
 %\cwu{introduce what serverless functions indeed are, and give example what serverless functions are used in MoE model inference}.


Current commercial serverless computing platforms (e.g., AWS Lambda \cite{Amazon}, Google Cloud Functions \cite{Google}, Azure \cite{Azure}, and Alibaba Cloud Functions \cite{Alibaba}) are CPU-based. % as CPUs are abundant and cost-effective.
Therefore, we focus on CPU-based serverless platforms in this paper.

%\cwu{introduce current commercial serverless computing platforms are CPU-based and we focus on CPU-based commercial serverless platform.}

\vspace{1mm}
\noindent\textbf{Function %deployment 
configuration.} Memory is the principal lever available to developers for controlling the performance of a serverless function. The memory configuration of a serverless function determines its computing speed, as more memory corresponds to more virtual CPUs %, enhancing computational power
\cite{Amazon}\cite{Google}. %\cite{Azure}\cite{Alibaba}. 
Users can configure the amount of memory to a serverless function and the serverless platform automatically allocates resources based on this configuration during function deployment. 
Commercial serverless computing providers \cite{Amazon}\cite{Google}\cite{Azure}\cite{Alibaba}%(e.g., Amazon\cite{Amazon}, Google\cite{Google}, Azure\cite{Azure}, and Alibaba Cloud\cite{Alibaba}) 
 generally charge users on the used memory during %the usage 
running time of a serverless function at the unit of GB-second (i.e., GBs). External storage and Docker image manager is charged on the size of stored objects, and severless function deployment manager usage is charged on the number of function invocations.
%Commercial serverless computing providers \cite{Amazon, Google, Azure, Alibaba}, %(e.g., Amazon\cite{Amazon}, Google\cite{Google}, Azure\cite{Azure}, Alibaba Cloud\cite{Alibaba}) 
%generally charge users as follows: for a serverless function, based on memory usage during running time of this functions in GB-seconds (i.e., GBs); for external storage and Docker image management, based on the size of stored objects; and for serverless function deployment management, based on the number of function invocations.
We focus on the billed cost of serverless functions as it represents % memory usage during running of functions is 
the primary %factor affecting 
cost %charges
for MoE model inference, %in serverless computing,
given a fixed model size and inference request workload. %This focus provides direct insights into cost efficiency and performance improvements. %for MoE model inference in serverless platforms.
%\cwu{more details of resource charging in serverless platforms, only charging serverless functions?}

%The serverless computing paradigm enables elastic cloud computing \cite{kounev2023serverless} for developing, deploying, and executing applications without the need to manage servers. Popular serverless computing providers, such as Amazon\cite{Amazon}, Google\cite{Google}, Azure\cite{Azure}, and Alibaba Cloud\cite{Alibaba}, implement elastic charging by providing Function as a Service (FaaS). 
%Such a function can elastically set its memory size for computing. When the memory size increases, the computation speed of the function is enhanced \cite{Amazon,Google,Azure,Alibaba}, because memory size determines the amount of available virtual CPUs in the function. With this observation, memory and time usage are associated with pricing in serverless computing platforms. In general, these providers bill users on the memory usage during the time of use at the unit of GBs. %\cwu{clarify what billed on GBs means, memory usage?}. 
%Therefore, there is a trade-off between cost and execution time when setting the memory of functions in serverless computing.
%Some limitations exist in the serverless function. First, the memory size of one serverless function is limited, leading to the adoption of external storage (e.g., S3 bucket in Amazon) to store large data (e.g., input, output, intermediate data, and model parameters) when not executing. %\cwu{clarify}. 
%For example, Amazon specifies the maximal function size of 10GB, Azure function is up to 1.5GB, and  Google and Alibaba Cloud maximally provide 32GB per function, while the parameter size of large models can reach hundreds of GB or even larger. Second, the transferred data size to invoke another function (termed {\em payload size}) is limited while the serverless function is stateless to retain no data, requiring transferring and processing all data once or adopting external storage to store the intermediate data.
%\cwu{not clear how the limited payload size is related to the serverless function being stateless, and communication relying on external storage. explain what the payload size is}. 
%With this observation, communication may rely on external storage for large data. For example, Amazon has the maximal payload size of 6MB, Azure function is up to 10MB, and  Google and Alibaba Cloud maximally allow one payload at 32MB.


%Hence, this paper focuses on minimizing the \textit{billed cost} of all \textit{MoE layers} for inference. Several reasons exist: first, if only inference time is optimized, setting all memory to the maximum suffices; then,  if only memory usage is optimized, the MoE model inference might take too long and fail to meet practical ML inference time limits; finally, since non-MoE layers resemble traditional ML models and can leverage existing designs, the focus is directed towards addressing the unique challenges of MoE layers.

\subsection{MoE Inference} 
%An MoE model adopts parallel expert structures to boost model capacity without adding computation. 
The gating network routes tokens to experts based on token features, %which refer to the token's inherent properties (
e.g., position in the inference request sequence, meaning of a word token, its roles in the sequence (subject, object, pronoun, verb, etc.) \cite{li2023accelerating}.  
This routing generally does not restrict the number of tokens to be processed by each expert, resulting in skewed popularity and unbalanced workloads among experts. GShard \cite{lepikhin2020gshard} enforces a threshold for the maximal number of tokens processed by one expert.
Zhou et al.~\cite{zhou2022mixture} %propose expert-choice routing, 
allow each expert to select the top-$k$ tokens and 
operate with a fixed bucket size.
Pre-gated MoE \cite{hwang2023pre} modifies the role of a gate function to preemptively %\cwu{proactively?} \mf{this paper use preemptively this word}
select the experts to be activated for the next MoE block. %to completely eliminate the sequential dependency between the expert selection and expert execution stage within any given MoE block. 
These proposals intervene in token-to-expert selection %i.e., change the algorithm
and hence may change model results \cite{lepikhin2020gshard, zhou2022mixture, hwang2023pre}. 
We do not modify token-to-expert routing decisions in our %serverless 
MoE inference serving.

\vspace{1mm}
\noindent\textbf{Distributed MoE inference.} %Serving MoE models in a distributed manner is essential due to the substantial computational demands of large-scale language models, which is largely carried out on GPU cluster because of GPU's high parallel-computing capability. For efficiency,
Expert parallelism is commonly adopted that allocates one device %(e.g., GPU) 
for each expert \cite{rajbhandari2022deepspeed}\cite{li2023accelerating}. %\cite{he2021fastmoe}\cite{zhai2023smartmoe}. 
For data parallelism in distributed MoE serving, each request batch is distributed across multiple devices %(e.g., GPUs) 
for simultaneous processing \cite{fedus2022switch}\cite{lepikhin2020gshard}. 
%\cwu{make sure the following includes a thorough survey of MoE serving works} 
%Besides data parallelism and expert parallelism \cite{rajbhandari2022deepspeed, fedus2022switch, lepikhin2020gshard, li2023accelerating, he2021fastmoe, hwang2023tutel},
%FastMoE \cite{he2021fastmoe} adopts expert parallelism and partition the MoE model to balance the workload \cwu{how they partition the MoE model and what workload they are balancing}. 
These parallelisms necessitate %all-to-all 
communication across multiple devices for input distribution and output aggregation. %in MoE layers; thus, some works \cite{rajbhandari2022deepspeed}\cite{xiong2022scomoe}\cite{singh2023hybrid} design a hierarchical method with intra-GPU, intra-machine, and inter-machine data transfers to reduce data transfer time between devices. %\cwu{why need this hierarchical all-to-all communication?} \cite{rajbhandari2022deepspeed}\cite{xiong2022scomoe}\cite{singh2023hybrid}. 
%Based on this hierarchical communication design, Chen et al.~\cite{chen2022highly} leverage the underlying memory structure of GPUs to overlap intra-node and inter-node communication in multi-GPU systems, resulting in faster communication. %\cwu{clarfy how it exploits the underlying memory structure to accelerate all-to-all further}. 
FasterMoE \cite{he2022fastermoe} applies tensor slicing and pipelining design to overlap all-to-all communication and computation in MoE layers. PipeMoE \cite{shi2023pipemoe} studies the pipeline degree for tensor slicing to adaptively pipeline communication and computation. %maximally hiding communication time and accelerating inference. 
MpipeMoE \cite{zhang2023mpipemoe} extends tensor slicing to multiple dimensions of the data, further expediting inference. The designs rely on the hardware architecture of GPU/CPU clusters, and thus cannot be adopted on serverless platforms. %\cwu{add a sentence to tell why their designs can not be adopted on serverless platform.} %All these works study MoE inference on traditional GPU clusters.

%\cwu{systematically survey and discuss any CPU-based MoE inference works and justify why CPU-based inference can be a good alternative (cost, performance).}
\begin{comment}
\cwu{the following are not pure CPU-based inference work so commented out to save space}
Due to the high cost and scarcity of GPUs, Huang et al.~\cite{huang2023towards} and Yi et al.~\cite{yi2023edgemoe} propose keeping popular experts in GPU memory and buffering the rest in CPU memory to reduce static memory allocation costs while maintaining performance. SE-MoE \cite{shen2022se} forms the CPU-GPU memory to load the model, and executes the computation tasks across the memory sections in a round-robin manner for efficient inference. Fiddler \cite{kamahori2024fiddler} use the computation ability of the CPU to minimize the data movement between the CPU and GPU, thereby accelerating in MoE inference. Given the low cost and abundant availability of CPUs, they can be used for MoE inference instead of GPUs and offer reliable performance, making CPU-based MoE inference a viable alternative. 
\end{comment}

\vspace{1mm}
\noindent\textbf{ML services in serverless platforms.} %\cwu{revise the following paragraph to discuss related work on DNN serving only, do exhaustive survey/discussion of serverless DNN inference works, and explain why serverless computing is beneficial for DNN serving and can meet DNN serving SLOs} 
% Training and inference of DNNs without the MoE architecture have been investigated on serverless computing platforms. 
% To accelerate DNN training, Feng et al.~\cite{feng2018exploring} propose hierarchical data transmission to reduce the communication time between serverless functions and external storage, and Wang et al.~\cite{jiang2021towards} redesign a communication method synchronizing model parameters in backpropagation (i.e., all-reduce) to expedite the communication.
% Wang et al.~\cite{wang2019distributed} apply deep reinforcement learning to produce a memory setup policy, and adopt data parallelism in training. 
% Funcpipe \cite{liu2022funcpipe} formulates a mixed integer quadratic program (MIQP) on the memory setup and serverless function replication problem, to optimize cost and execution time for distributed training with data parallelism and model partition.
% To minimize the cost of ML inference on serverless computing platforms, Amps-inf \cite{jarachanthan2021amps} partitions the model through a mixed integer quadratic program (MIQP), and Ali et al.~\cite{ali2020batch} design a batch queue for request batching. 
Extensive research has focused on optimizing ML model serving in serverless platforms. Amps-inf \cite{jarachanthan2021amps} studies model partitioning to minimize inference costs. %For batching, 
Ali et al.~\cite{ali2020batch} design a request batch queue to reduce costs, while INFless \cite{yang2022infless} reduces inference latency %and enhances throughput 
by optimizing batch queuing, execution time, and cold start rates. %Regarding memory efficiency, INFaaS \cite{romero2021infaas} offers an automated system for generating model variants from pre-trained models, while TETRIS \cite{li2022tetris} designs a memory-efficient serverless runtime through tensor sharing. 
Gillis \cite{yu2021gillis} adopts model partitioning and scheduling for low-latency large DNN model inference, while ServerlessLLM \cite{fu2024serverlessllm} focuses on fast multi-tier checkpoint loading and optimized startup-time scheduling. %Serverless computing is promising for
DNN serving on serverless platforms has been proven effective in meeting serving SLOs and %allows dynamic scaling to efficiently 
handling %large models and 
varying workloads.
However, there is a lack of designs for efficient MoE inference on a serverless platform. 
 %\mf{LambdaML does not focus on MoE model inference in serverless platforms. It is still just an over-provisioning method many works commonly use. It is a void field after I verified in 30/07/2024. Only some surveys suggest serverless MoE inference can be a future topic.}
 %To our knowledge, LambdaML \cwu{cite} is the first to optimize the distributed deployment of MoE model inference in serverless platforms \cwu{briefly dsicuss this work and any other works on MoE inference on a serverless platform}. 

\subsection{Opportunities and challenges}
\begin{figure}[!t]
\centerline{\includegraphics[width=0.48\textwidth]{evaluation_figs/cpu_throughput.pdf}}
\vspace{-3mm}
\caption{Billed cost of all MoE layers and inference throughput of a GPT-2-based MoE model. %for 10,240 tokens from the Enwiki8 dataset on CPU clusters and AWS Lambda. 
%\cwu{remove `Platforms from the figure; change Serverless Computing to AWS Lambda}
}
\label{fig_cpu_throughput}
\vspace{-5mm}
\end{figure}
\noindent\textbf{Opportunity: MoE model inference in a serverless platform can bring substantial cost reduction and satisfactory inference performance}, as compared to CPU cluster-based inference serving. %Serverless frameworks provide new opportunities to reduce the cost of ML model inference in comparison with MoE serving on traditional CPU clusters, due to 
On a serverless platform,  %Memory size of serverless functions can be elastically set, benefiting workload-imbalanced, distributed MoE models. 
%In Fig.~\ref{ServerlessComputing},
expert networks can be individually assigned to serverless functions with different memory size configurations, so that more resources are rent for workload-heavy experts and less for workload-light experts. %during model serving. 
Further, inference functions are invoked on-demand at fine-grained timescales (i.e., milliseconds) \cite{Amazon}\cite{Google}.%\cite{Azure}\cite{Alibaba}. 
Serverless functions %of an expert
are only billed on assigned memory when executing; no cost for idle resources is incurred. However, the cost of a CPU cluster typically depends on the amount of resources over a fixed coarse-grained period (e.g., per month or per hour), so that costs may still be incurred for idle resources.
%For example, 
Fig.~\ref{fig_cpu_throughput} shows the billed cost of all MoE layers and inference throughput, when a GPT-2-based MoE model serves 10,240 tokens from the Enwiki8 \cite{enwik8} dataset. %\cwu{cite the dataset}. %in CPU clusters and AWS Lambda. 
The CPU cluster uses two 64-core AMD EPYC CPUs with 512GB of DRAM for the entire MoE model. %\cwu{briefly tell the CPU cluster configuration - what CPUs are used}. %while AWS Lambda employs expert parallelism, and each expert, each non-MoE layer combined with the subsequent gating network, and the final MoE layer are each assigned to separate serverless functions, 
Each serverless function for MoE inference on AWS Lambda is allocated 3008 MB of memory. The billed cost of all MoE layers on AWS Lambda is significantly lower than on the CPU cluster. The throughput of MoE inference on the serverless platform is 22.9 tokens per second, substantially exceeding the human reading speed of 3.3 tokens per second \cite{kotani2011machine}. %\cwu{add citation}. 
Hence, serverless-based MoE inference presents a viable solution.
Two challenges exist on enabling efficient deployment and serving of an MoE model on a serverless platform.

\begin{figure}[!t]
\centerline{\includegraphics[width=0.45\textwidth]{figs/real_token_ID.pdf}}
\vspace{-3mm}
\caption{Number of tokens with token ID 10424 (from the Enwiki8 dataset) routed to different experts at the 2nd MoE layer in Bert-based MoE model.%  on AWS Lambda. 
%\cwu{label integer numbers on the horizontal axis}
}
\label{fig_tid}
\vspace{-5mm}
\end{figure}

\vspace{1mm}
\noindent\textbf{Challenge 1: Skewed, unknown-beforehand expert popularity prevents proactive, accurate memory configuration of serverless functions.} Expert selection is %decided by the routing results of the gating network during inference serving, 
unknown before actual token processing by the gating network. 
Dynamic resource allocation, %\cwu{explain what this dynamic resource allocation does}
which decides computational resources for each expert based on real-time expert popularity during inference, has been advocated for MoE serving in GPU/CPU clusters \cite{he2021fastmoe}\cite{he2022fastermoe}. %In a serverless platform, 
Serverless functions require a long time to deploy (e.g., 1 minute or longer) and to start execution (e.g., 5 seconds or longer) %for the first time 
after deployed \cite{zhang2021caerus}; 
%i.e., the cold start issue 
on-demand dynamic function redeployment is largely infeasible, which would substantially slow down inference serving. This necessitates %proactive function deployment with 
proper configuration of memory sizes when deploying serverless functions before service starts, requiring prior knowledge of expert popularity. Improper memory configuration may either fail to meet the memory demand during inference, or %excessive memory can result in 
incur higher billed costs due to unnecessary memory usage.
FlexMoE~\cite{nie2023flexmoe} and Prophet~\cite{wang2023prophet} use average historical expert popularity %as the estimate
to adjust resources among experts.
Lina~\cite{li2023accelerating} predicts expert popularity before model deployment using the maximum a posteriori probability based on historical %data, and the historical data records a 
token-to-expert mapping and token ID information. %is identified by the unique numerical identifier (i.e., token ID) assigned by a predefined vocabulary. %\cwu{clarify how they predict expert selection through probability} before deploying the model. 
Cong et al.~\cite{cong2024prediction} propose an LSTM-based algorithm trained on historical token-to-expert mapping for expert selection predication.
These expert selection prediction methods %have have drawbacks: some algorithms 
may achieve low prediction accuracy as the token-to-expert relationship %distribution \cwu{what is token distribution?} 
in historical data is not exploited 
~\cite{nie2023flexmoe,wang2023prophet}, %, while some algorithm has a high accuracy but 
or are memory-intensive and require a long training time~\cite{cong2024prediction}. Lina~\cite{li2023accelerating} considers the token distribution %in token-to-expert mappings in historical data without memory intensity 
but only uses token ID as the token feature.
%\cwu{discuss all expert selection prediction works here; discuss works advocating "replicating popular experts" (FasterMoE?) and why it is not suitable in serverless platform}. \mf{"replicating popular experts" is also a dynamic allocation network} \cwu{discuss insufficiency of the above expert selection prediction methods}. 
%Accurately predicting expert popularity is challenging due to limited available information \cwu{clarify why the available information is limited}, such as basic inputs only with token IDs.
Token ID is insufficient to fully identify a token in token-to-expert mappings, as tokens with the same token ID may be routed to different experts at a MoE layer, as illustrated in Fig.~\ref{fig_tid}. %However, before inference, only the token ID is available, while more information about the token becomes available only during the inference process and cannot be obtained beforehand. Hence, accurately predicting expert popularity is challenging.

 \begin{figure}[!t]
 \centering
 \subfigure[256 tokens]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/communication_cost_latency_token256.pdf}}
 \subfigure[2560 tokens]{
\includegraphics[width=0.23\textwidth]{evaluation_figs/communication_cost_latency_token2560.pdf}}
\vspace{-3mm}
 \caption{Billed cost of all MoE layers %\cwu{what MoE model on what serverless platform and tokens from what dataset} 
 and end-to-end inference time of a Bert-based MoE model on AWS Lambda (tokens from Enwiki8 dataset; %under direct and indirect MoE scatter-gather communications. Note that 
 payload size 6MB %\cwu{inconsistent with discussion text - give the payload size in this experiment}
 ).
 }
\label{motivation_alltoall}
\vspace{-5mm}
\end{figure}

\vspace{1mm}
\noindent\textbf{Challenge 2: MoE scatter-gather communication renders performance bottlenecks in serverless MoE inference.} 
In each MoE layer, scatter communication occurs between the gating network and expert networks, and gather communication between expert networks and the subsequent non-MoE layer,
which often renders a bottleneck  %that blocks subsequent operations %during inference \cite{singh2023hybrid}\cite{shi2023pipemoe}. 
because the non-MoE layer must wait for all experts to complete their computation and communication. %introducing additional delays and blocking subsequent operations.
%\cwu{discuss more and clearly why existing all-to-all communication optimization in traditional GPU/CPU cluster (as discussed in "Distributed MoE model inference" part) is not applicable in serverless platforms.}
%Unlike in GPU/CPU clusters, direct communication between serverless functions is limited by the platform-specified payload size, and indirect data transfers via the external storage are often needed. 
The direct and indirect inter-function communication on a serverless platform results in different billed costs and inference time. 
In Fig.~\ref{motivation_alltoall}, MoE scatter-gather communication via indirect transfers incurs higher cost %which depends on memory usage and running time
and longer inference time than direct transfers when serving a 256-token batch, due to the additional function running time required for storing data in external storage and retrieving data as input. 
Direct transfers cannot be adopted when serving a 2560-token batch as the payload size is exceeded; %between serverless functions assigned as experts and serverless function assigned as non-MoE layer with the subsequent gating network. 
the serving cost under indirect transfers is very high. 
While pipelining communication with computation can typically alleviates this bottleneck in GPU/CPU clusters, 
pipelining in a serverless platform needs to take its direct or indirect data transfer modes into consideration, and carefully designed to improve efficiency in a serverless platform. %mitigating its bottlenecking in MoE model inference.%Direct communication is incompatible with pipelining because serverless functions are stateless, and direct data transfers require re-invocation each time, preventing the retention of model parameters during transfers and leading to wasted time and memory for loading parameters without inference computation; indirect transfers, which rely on external storage, add complexity to pipelining design.
\begin{comment}
\cwu{show all-to-all communication time in the end-to-end inference time, cost incurred by all-to-all communication time in overall cost, to give readers clear idea that it renders the bottleneck.}\mf{I'll run this experiment in 30/07/2024.}
\end{comment}


We redesign token features and propose a novel posterior calculation method for expert selection prediction. %and an adjustable key-value dataset table in terms of expert selection prediction. 
We design and select the best scatter-gather communication methods for MoE layer inference.
We involve all modules in a BO framework for optimal MoE serving deployment.


==> Sec3-Design.tex <==
\section{Design}\label{Secdesign}


\subsection{System overview}\label{systemoverview}
We consider distributed deployment of an MoE model in a serveless computing platform to serve inference requests. %The serverless platform includes serverless functions, external storage, Docker image manager, and serverless deployment manager. 
The MoE model consists of MoE layers (each includes a gating network and multiple experts) and non-MoE layers (e.g., feed-forward networks, multi-head attention networks \cite{fedus2022switch}). %In this paper, 
We adopt expert parallelism \cite{rajbhandari2022deepspeed, li2023accelerating} by assigning each expert to a serverless function. Model parallelism is adopted for non-MoE parts of the model with each non-MoE layer %and the subsequent gating network in a MoE layer are 
assigned to a serverless function. Model parameters are store in external storage.
%each model part is built as a Docker image stored in Docker image manager, and each Docker image create a serverless function.
We mainly focus on the MoE layers %in serverless computing 
since the non-MoE layers are traditional DNNs extensively studied \cite{yu2021gillis} \cite{romero2021infaas}.
% We consider distributed deployment of an MoE model in a serveless computing platform to serve inference requests. The serverless platform includes xx \cwu{give system overview of the serverless platform}. 
% The MoE model consists of MoE layers (each includes a gating network and multiple experts) and non-MoE layers (e.g., \cwu{give example non-MoE layers in an MoE model}). The MoE model is partitioned using xx and expert parallelism \cwu{tell what data or model or expert parallelism you are assuming to run the MoE model}. \cwu{Each non-MoE layer and each expert in each MoE layer?} are run as a serverless function, respectively, where each function can run as multiple distributed instances on the serverless platform.  
%The MoE model deployment is periodically adjusted to best serve varying inference requests, with proactive expert deployment according to expert popularity predictions on the go. The goal is to minimize overall billed cost of all MoE layers in serving.

We propose a %carefully designed 
Bayesian Optimization (BO) framework to learn expert selections and optimal deployment of the MoE model for inference serving. The goal is to minimize overall billed cost of all MoE layers in serving. The BO framework consists of  
a {\em Feedback Processor} to adjust expert selection prediction, an {\em Expert Selection Predictor}, and a {\em Policy Maker}. 
An illustration is given in Fig.~\ref{sysoverview}. 
%We assume the MoE layers are distributed based on expert parallelism, with each expert occupying at least one serverless function.
%We assume data parallelism is applied to the entire MoE model and the MoE layers are distributed based on expert parallelism 
%Here replicating the entire model but not just the non-MoE model serves for the pipeline design in all-to-all communication introduced later. 
%The entire MoE model is replicated to handle split data and each expert occupies a serverless function. %entire MoE model is replicated 
%as %\cwu{clarify the idea of the following, whats the difference between serverless functions and the new function? How exactly is stateless property relevant}
%multiple serverless functions cannot directly integrate the intermediate outputs into another function multiple times before these functions finish this execution to enable pipeline data transfer operation. 
%In serverless computing, integration of multiple functions directly to another function can only happen after these functions finish this execution (i.e., step function deployment).
%due to the stateless property impeding the invoked function retaining the data to accept a new invocation. Dashed lines represent the all-to-all communication around the MoE layers. %The MoE model is deployed in serverless computing with the assistance of an expert selection predictor, a policy maker, and an overall processor. 
The expert selection predictor provides expert predictions of inference tokens from a real-world dataset on an inference task. This prediction is based on the posterior distribution calculated from these tokens and profiled data. The profiled data records the number of times each token-to-expert mapping occurs across at least 100 samples from the same real-world dataset, %in the same inference task of the same MoE model in advance, 
organized in a key-value dataset table. %where the keys represent token-to-expert mappings and the values denote their occurrence counts. A token is represented by our carefully designed token features, and an expert is identified by its index. The profiled data can, to some extent, represent token-to-expert mapping distributions in actual inference serving because it captures the underlying patterns from historical samples in the same MoE inference process. 
With the predictions, the policy maker decides how to deploy the MoE model, configures the memory size of each expert serverless function and adopts our scatter-gather communication design. 
The feedback processor adjusts the key-value pairs in the profiled dataset table for improving expert selection prediction, using feedback of the billed cost of all MoE layers in serving. In each BO iteration, expert predictor is adjusted, the policy maker decides optimal deployment of the MoE model, and the billed cost is collected for feedback processor's key-value table adjustment. %until the real billed cost decreases little (i.e., achieving convergence of BO). After the convergence in an adjustment, the feedback processor identifies the optimal key-value pairs for expert predictor that minimizes real billed cost. In the first period to adjust, the feedback processor collects real billed cost on a open-source real-world dataset and different real-world dataset is used for different tasks. In the following periods, the billed cost is obtained based on the inference requests from real-world datasets encountered after the last adjustment. After each adjustment, the feedback processor becomes inactive and the adjusted expert predictor works with the policy maker for inference requests before from the real-world dataset the MoE deployment. %With the prediction results, the policy maker decides how to deploy the entire MoE model, sets the memory size of each expert serverless function and adopts our all-to-all communication design. 

When the BO algorithm converges, %is done offline with a real deployment by feedback processor to obtain a converged optimal adjusted expert predictor, and then 
the MoE model is deployed according to the learned expert popularity and optimal deployment policy, and serves real-world inference requests.


%runs on sampled token features and their expert selection results

% \cwu{rewrite the following to clearly how you get the data for BO - how do you get the sampled batches of tokens and their expert selection results? tell about using different open-source real-world dataset for different tasks and justify why they can represent token distributions in actual inference serving: from at least 100 sampled batches of tokens and their expert selection results in each MoE layer in advance}. 
% The profiled data is stored in a key-value %dataset 
% table, where the %primary 
% key consists of token features and indices of selected experts, and the value is the number of tokens satisfying the primary key criteria \cwu{what does `satisfying the primary key criteria' mean? the tokens with the feature and expert selection specified in the key?}.  


% The expert selection predictor provides expert selection prediction results of tokens in new inference requests \cwu{clarify what the `new data' is referring to}, based on token information. With the prediction results, the policy maker decides how to deploy the entire MoE model, sets the memory size of each expert serverless function and adopts our all-to-all communication design. The deployment is then adjusted according to policy maker's decisions, and the MoE model processes inference request; the billed cost of model serving is provided as feedback to the feedback processor. The feedback processor fine-tunes the key-value table %$\mathcal{D}(\cdot)$ can be adjusted
% by modifying an existing key's value \cwu{how to modify?} or adding a new key-value pair \cwu{what new key-value pair to add? how the feedback is used?}. This changes the profiled probabilities for expert selection predictor to compute the expert selection again. %improving the accuracy of expert predictions using a Bayesian decision-making policy. As a result, a better optimal deployment policy may be obtained, minimizing the billed cost of all MoE layers. The finetuning process is guided by the actual billed cost of all MoE layers. %the overall processor stops trails to update new data patterns, and 
% %After finetuning, the expert selection predictor can provide better prediction results for future inference executions.

% \cwu{tell that when the BO algorithm converges(?), the MoE model is deployed in the serverless platform according to the converged optimal deployment strategies, and used for inference serving. Tell if the BO algorithm is done offline without real deployment or otherwise}


\begin{comment}
For notations, let $\mathbb{X}$ represent a set, $\mathbf{x}$ represent a vector, $x$ represent a scalar, and $\mathcal{X}(\cdot)$ represent a function. $|\mathbb{X}|$ denotes the cardinality of the set $\mathbb{X}$. Subscripts of $x$ indicate positions in the set, such as $x_{e,i}$ with $i\in\mathbb{N}_e$ and $e\in\mathbb{E}$. Superscript denotes roles of a variable, such as $x^{h, NE}$ indicating $x$ at the head of a non-MoE layer. 
Except for indices, sets and Greek letters, lowercase letters $x$, $\hat{x}$ and $\tilde{x}$ represent unknown variables, and and uppercase letters $X$ represent knwon values. $x^*$ denotes $x$ from profiled data while $x'$ denotes $x$ from new data.
%Notations are shown in Table~\ref{tab1}.
\end{comment}

\begin{figure}[!t]
\centerline{\includegraphics[width=0.45\textwidth]{figs/Visio-system_overview.pdf}}
\vspace{-3mm}
\caption{System Overview. %\cwu{why there are two non-MoE layer 1?}
%\cwu{correct the specification of non-MoE layers, draw more realistic MoE model with MoE and non-MoE layers with assumed parallelism; also, is it common for one gate network to follow the experts? i.e., consecutive MoE layers in an MoE model?}.\mf{yes, it is common}
%\cwu{Merge Fig. 3 into this Figure by replacing the MoE model part in the figure}
}
\label{sysoverview}
\vspace{-5mm}
\end{figure}

%For the rest of this paper, we introduce the principles of system design, including expert selection prediction in \hyperref[Secdesign]{SecIII.B}, all-to-all communication design and deployment formulation for the policy maker in \hyperref[Secdesign]{SecIII.C} and \hyperref[Secdesign]{SecIII.D}, and the algorithm for the overall processor to finetune the expert predictor in \hyperref[secAlg]{SecIV}. Finally, we evaluate the performance in \hyperref[Secevaluation]{SecIV}.

\iffalse
\begin{table}[!t]
\begin{center}
\caption{Notation %\cwu{the table should occupy the whole column width; the first column of the table can occupy less width and the second occupy more}
}
\vspace{-3mm}
\begin{tabular}{|p{1.4cm}|p{6.5cm}|}%\toprule
\hline
\small
${\bf f}$ &  token feature \\\hline
$\mathbb{E}$ & set of MoE layers indices\\\hline
$\mathbb{M}$& set of memory size options\\\hline
$\mathbb{N}_e$ & set of experts indices in MoE layer $e$ \\\hline
$\mathbb{G}_{e,i}$ & set of replication number options for expert $i$ at MoE layer $e$ \\\hline
$d_{e,i}$ & number of tokens routed to expert $i$ in MoE layer $e$ from the previous non-MoE layer \\\hline
$r_{a_e, e,i}$ & number of tokens routed to one replica of expert $i$ in MoE layer $e$ from the previous non-MoE layer under communication method $a_e$ \\\hline
$U_j$ & unit computation time given memory type $j$\\\hline
$s_{e,i}$ & if expert $i$ will be routed (1) or not (0) in MoE layer $e$ \\\hline
$P_{e,i}$ & parameter size of expert $i$ in MoE layer $e$ \\\hline
$R_{e,i}$ & intermediate activation size of expert $i$ in MoE layer $e$\\\hline
$D^{in}$ / $D^{o}$ & one token size / output size of one token as input in inference \\\hline
$w_{e,i}$ & workload of expert $i$ in inference for one token in MoE layer $e$\\\hline
$t^{load}_{e}$ & warm start and download model time of next non-MoE layer of MoE layer $e$\\\hline
$t^{cal,NE}_{e}$ & calculation of previous non-MoE layer of MoE layer $e$\\\hline
$T^{head}$ & execution time of first non-MoE layer without calculation and data transfer time \\\hline
$T^{tail}$ & execution time of last non-MoE layer without model download and data receiving time \\\hline
$T^{limit}$ & time limit of inference with one batch of input request\\\hline
$B^s / B^f$ & bandwidth between external storage / function and function \\\hline
$T^{str}$ & warm start time of serverless function\\\hline
$T^{dl}$ & access delay to external storage\\\hline
$D^p$ & payload size limit \\\hline
$a_e$&if the all-to-all communication uses pipelined indrect transmission (1), unpipelined indirect transmission (2) or direct transmission (3) \\\hline
$\beta$ & number of tokens in a scattered block to communicate \\\hline
$x_{a_e,e,i,j}$ & if the expert $i$ selects $j$-memory size option (1) or not (0) in MoE layer $e$ \\\hline
$y_{a_e,e,i,g}$ & if the expert $i$ has $\mathbb{G}_{e,i,g}$ replications (1) or not (0) in MoE layer $e$
\\\hline

\end{tabular}
\label{tab1}
\end{center}
\vspace{-5mm}
\end{table}
\fi

\subsection{Expert selection prediction}\label{expertselection}

% In the MoE model, each token in an inference request is routed to top-$k$ experts by the gating network in each MoE layer. 
% The routing rule of the gating network is typically decided by the token's inherent properties (e.g., position in the inference request sequence, %\cwu{inference request sequence?}, 
% meaning of a word token \cite{li2023accelerating}) and its roles in the token sequence (e.g. subject, object, pronoun and verb), %\cwu{clarify what the roles in the token sequence mean}, 
% referred to as the token features. %Given the token features, we seek to make expert selection prediction of each token before distributed deployment for MoE model inference. Two issues should be tackled, namely the prediction approach and the token feature choice.

In an MoE model, each token in an inference request is routed to top-$k$ experts by the gating network at an MoE layer, based on token features. %such as position in the sequence, meaning of the word token, and its grammatical role (e.g., subject, object, pronoun, verb) \cite{li2023accelerating}. These token-to-expert mappings can be recorded as profiled data, aiding in expert selection prediction for the same MoE model and serving task \cite{li2023accelerating, cong2024prediction}. A token is typically represented by its token features, like token ID \cite{li2023accelerating}. However, the 
Token ID is the most commonly used token feature \cite{li2023accelerating}, but itself alone is insufficient to fully identify a token in token-to-expert mapping. We carefully design token features %to better represent a token 
by investigating more token information during MoE inference. As Transformer models are typically the backbone of MoE models \cite{fedus2022switch}, we focus on Transformer-based MoE models.


% \cwu{How is the following discussion of different token features related to S's computation above?}
% Other than token ID, we choose more token features to capture additional information about processed tokens before they are routed by the gating network.
% %\cwu{not clear why the following sentence is related to token feature selection} the token processing can be investigated in the MoE model inference. 
For Transformer-based MoE models, token processing mainly occurs in the embedding, encoder and decoder layers. In the embedding layers, each token is embedded with its own information and its position (e.g., word embedding and position embedding). Thus, the token ID and position ID can be extracted as token features. In the encoder and decoder layers, tokens flow through feed-forward networks and one multi-head attention. In the feed-forward networks, no dependencies exist within the token sequence, so token ID and position ID are sufficient as the token features. 
Each multi-head attention layer contains multiple self-attentions. Each self-attention calculates the Query, Key, and Value of the tokens to capture dependencies between tokens in the token sequence.  The dependencies are quantified by the softmax attention scores, which indicate the relevance of each token to the others. For each token, we extract these dependencies as a token feature.
For simplicity, the dependencies for each token are derived as the token ID of the token with the highest sum of softmax attention scores across all self-attentions at a multi-head attention layer, referred to as the attention ID. %\cwu{only the token with the highest sum of softmax attention scores has an attention ID or each token has such an attention ID?}.
% Through the Query and Key,the softmax attention score of each token can be obtained to represent its relevance to other tokens in the sequence. Therefore, softmax attention scores should be profiled as token features. However, each token corresponds to multiple softmax attention scores across self-attention layers. %\cwu{not clear what `combine with related probabilities of token' means}, 
% For simplicity, we use the token ID of the token with the highest sum of softmax attention scores across all self-attentions at a multi-head attention layer before a MoE layer for each token, referred to as the attention ID. 
The attention ID may vary before different MoE layers, aligning with the diverse expert popularities at different MoE layers. %of the same MoE model processing the same tokens observed in practical implementations. 
Therefore, the token features include the token ID, the position ID, and the attention ID. The token IDs and position IDs are from the input token sequences, known before inference starts. The attention IDs are from the self-attention parts of the non-MoE layer before each MoE layer, known during inference. 

%With these token features, we can identify a token in the token-to-expert mapping in the profiled data.
%For a serving task in an MoE model,
Our expert prediction in the BO framework is learned on profiled data, which records the token-to-expert mappings on at least 100 samples from a real-word dataset of inference task. The profiled data are organized in a key-value dataset table where the keys represent token-to-expert mappings and the values denote their occurrence counts.
%For tokens that have not yet undergone this MoE inference task in this real-world dataset, the key-value dataset table can be used to decide the selected expert based on their token features, typically using a maximum posterior method where the posterior represents the probability of an expert given a token \cite{li2023accelerating}. This requires the token features of these tokens are obtained before inference, easy for token IDs. For the position IDs, if the order of token sequences is known, each token can obtain its position ID; otherwise, each token cannot know its position ID but the probability of position IDs at any value is uniform without considering specific tokens. The attention IDs, defined as the token ID with the highest sum of softmax attention scores, requires inference but are related to known token IDs. Hence, 
Especially, we design a new posterior calculation method and use the maximum posterior approach to predict expert selection for new tokens, where the posterior represents the probability of an expert given a token \cite{li2023accelerating}. %that have not yet undergone MoE inference.
 %\cwu{at all the multi-head attention layers?} 
 % The multi-head attention layers before different MoE layers yield varying expert selection results, aligning with the diverse expert popularities at different MoE layers observed in practical implementations. %\cwu{not clear what practical situations are referring to here}. 
 % With these token features, we can distinguish tokens routed to different experts at each MoE layer, enabling the expert selection prediction for new tokens.%\cwu{clarify in this paragraph what features are from non-MoE layers before gating network, what are features from MoE layer and why we need MoE layer features to make the prediction.}


Assume ${\bf f}$ is the token feature vector of a token, in which ${\bf f}_1$ is the token ID, ${\bf f}_2$ is the position ID and ${\bf f}_3$ is the attention ID. The posterior given the token can be expressed as $\mathcal{P}(\mathbb{N}_{e,i}|{\bf f})$ with $e\in\mathbb{E}$, where $\mathbb{N}_{e,i}$ is the $i$-th expert in the expert set $\mathbb{N}_{e}$ at MoE layer $e$ and $\mathbb{E}$ is the set of MoE layers in the MoE model. For a new token %from the tokens in a real-world dataset 
that has not undergone MoE inference, 
its feature ${\bf f}'_1$ is known but ${\bf f}'_3$ is unknown, %before inference, and ${\bf f}'_3$ cannot be obtained assuming the order of token sequences are unknown. 
The probability of ${\bf f}_2$ at any position is uniform, and the probability of ${\bf f}_3$ at any value can be approximated by the probability of ${\bf f}_1$ at that value, as the attention ID ${\bf f}_3$ is defined as the token ID with the highest attention scores. We can obtain all probabilities related to ${\bf f}'_1$ from the profiled data, %on the same real-world dataset in the same MoE serving task, 
the uniform probability $\mathcal{P}'({\bf f}_2)$ of ${\bf f}_2$ at any value and the probability $\mathcal{P}'({\bf f}_3)$ of ${\bf f}_3$ at any value from tokens in the same real-world dataset, that have not undergone MoE inference. %where $\mathcal{P}'(\cdot)$ denotes the probability calculated from the tokens that have not yet undergone MoE inference.

To leverage all token features for identifying a token effectively, we use Bayes' theorem to design a new posterior calculation method. The Bayes' theorem $\mathcal{P}(\mathbb{N}_{e,i}|{\bf f})=\mathcal{P}({\bf f}|\mathbb{N}_{e,i})\mathcal{P}(\mathbb{N}_{e,i})/\mathcal{P}({\bf f})$ describes how the posterior of an expert selection given a token $\mathcal{P}(\mathbb{N}_{e,i}|{\bf f})$ is updated with the prior of the expert $\mathcal{P}(\mathbb{N}_{e,i})$, the prior of the token $\mathcal{P}({\bf f})$, and the likelihood of the token given the expert $\mathcal{P}({\bf f}|\mathbb{N}_{e,i})$. As $\mathcal{P}(\mathbb{N}_{e,i}|{\bf f}'_1)=\mathcal{P}({\bf f}'_1|\mathbb{N}_{e,i})\mathcal{P}(\mathbb{N}_{e,i})/\mathcal{P}({\bf f}'_1)$ and $\mathcal{P}({\bf f}'_1|\mathbb{N}_{e,i})=\mathcal{P}({\bf f}'_1,\mathbb{N}_{e,i})/\mathcal{P}(\mathbb{N}_{e,i})$, we can involve the uniform probability $\mathcal{P}'({\bf f}_2)$ of ${\bf f}_2$ and the probability $\mathcal{P}'({\bf f}_3)$ of ${\bf f}_3$ into the likelihood $\mathcal{P}({\bf f}'_1|\mathbb{N}_{e,i})$ of the expert given ${\bf f}'_1$, through the joint probability $\mathcal{P}({\bf f}'_1,\mathbb{N}_{e,i})$. For simplicity, we multiply $\mathcal{P}'({\bf f}_2)$ and $\mathcal{P}'({\bf f}_3)$ with $\mathcal{P}({\bf f}'_1,\mathbb{N}_{e,i})$ as involvement. Hence, the designed posterior calculation method is given by:
\begin{equation}\label{Byderive}
\small
\begin{aligned}
       \mathcal{P}(\mathbb{N}_{e,i}|{\bf f}'_1)
        = \int_{{\bf f}_{2}}&\int_{{\bf f}_{3}}\mathcal{P}^*(\mathbb{N}_{e,i}|{\bf f}'_1,{\bf f}_{2},{\bf f}_{3})\frac{\mathcal{P}^*({\bf f}'_1,{\bf f}_{2},{\bf f}_{3})\mathcal{P}'({\bf f}_{3})}{\mathcal{P}^{*}({\bf f}'_1,{\bf f}_{2})}d{\bf f}_{3}\\
        &\frac{\mathcal{P}^*({\bf f}'_1,{\bf f}_{2})\mathcal{P}'({{\bf f}_2})}{\mathcal{P}^{*}({\bf f}'_1)}d{\bf f}_{2}, \forall e \in \mathbb{E}, \forall i \in \mathbb{N}_e,
\end{aligned}
\end{equation}

where $\mathcal{P}^*(\cdot)$ represents the probability calculated from profiled data in the key-value dataset table.

Therefore, we can use the maximum a posterior method to predict the expert selection for a token with the known token feature ${\bf f}'_1$:

\vspace{-5mm}
\begin{equation}\label{ideaby}
    \small
    \hat{i}_{e}=argmax_{i\in\mathbb{N}_e} \mathcal{P}(\mathbb{N}_{e,i}|{\bf f}'_1), \forall e \in \mathbb{E},
\end{equation}
where $\hat{i}_{e}$ is the predicted expert at MoE layer $e$. Eq.~(\ref{ideaby}) can be readily extended to top-$k$ expert selection prediction.

%The expert selection prediction can be adjusted by changing the key-value pairs in the dataset table, as the probabilities are calculated from the values in the dataset table and then used in the designed posterior calculation method.



% %For the prediction approach,  Inspired by \cite{li2023accelerating}, 
% We calculate the probability of expert selection of each token for expert popularity prediction. 
% Unlike direct use of profiled posterior probability for new data \cwu{clarify what the profiled posterior probability for new data means and cite which existing work directly uses this profiled posterior probability for prediction?}, we further consider the probability of token features in new data \cwu{clarify what the probability of token features in new data means}, which is often the only available information \cwu{why it is the only information, what about token ID, roles, etc., as you mentioned among token features?}, and combine this probability with the profiled posterior to obtain a %adjusted 
% new posterior. %Based on this, for top-$k$ MoE model, 
% We decide the $k$-th expert $\hat{i}_{k,e}$ at MoE layer $e$ for a new token with token feature ${\bf f}'$, by maximizing this new posterior probability:
% \begin{equation}\label{ideaby}
% \begin{aligned}
%     \small
%     \hat{i}_{k,e}&=argmax_{i\in\mathbb{N}_e} \mathcal{S}_{k,e,i}({\bf f}'),
%     \forall k\in \mathbb{K}, \forall e \in \mathbb{E},
% \end{aligned}
% \end{equation}
% where $\mathcal{S}_{k,e,i}({\bf f}')=\mathcal{P}(\mathbb{N}_{e,i}|\mathbf{f}')$ denotes the new posterior function for the $k$-th expert $i$ at MoE layer $e$. %$e\in\mathbb{E}$ denotes the MoE layer $e$ in 
% $\mathbb{E}$ is the set of MoE layers in the MoE model, % $i\in\mathbb{N}_e$ represents the expert $i$ in 
% $\mathbb{N}_e$ is the expert set at MoE layer $e$, and %$k\in \mathbb{K}$ represents the $k$-th expert selection for a token in 
% $\mathbb{K}$ is the index set of top-$K$ experts. 
% \cwu{explain $\mathbb{N}_{e,i}$.}

% %The function 
% $\mathcal{S}_{k,e,i}({\bf f}')$ is constructed based on Bayes' theorem \cwu{tell what the Bayes' theorem is like or does}, describing how the posterior is updated with the prior, likelihood, and evidence \cwu{explain which of the following quantities correspond to prior, likelihood, and evidence}. Suppose token feature ${\bf f}$ has $H$ dimension. $\mathcal{S}_{k,e,i}(\mathbf{f}')$ is computed in three steps:
% (1) we individually compute the joint probability %$\mathcal{P}(\mathbb{N}_{e,i}, \mathbf{f}'_h)$ by 
% $\mathcal{P}(\mathbb{N}_{e,i}, \mathbf{f}'_h)=\mathcal{P}^*(\mathbb{N}_{e,i}, \mathbf{f}')\mathcal{P}'(\mathbf{f}')$, where $\mathcal{P}^*(\cdot)$ is the profiled probability, $\mathcal{P}'(\cdot)$ denotes the probability of new data, and $\mathbf{f}'_h$ represents xx \cwu{explain}, $\forall h\in\{1,\dots,H\}$. (ii) We %rewrite the joint probability $\mathcal{P}(\mathbb{N}_{e,i}, \mathbf{f}')$ by 
% then iteratively compute $\mathcal{P}(\mathbb{N}_{e,i}, \mathbf{f}'_{1:h})=\mathcal{P}(\mathbb{N}_{e,i}, \mathbf{f}'_{h-1})\mathcal{P}^*(\mathbf{f}'_{h-1}|\mathbb{N}_{e,i}, \mathbf{f}'_{1:h-2})$ %until 
% \cwu{for $h=1, \ldots, H$?}, where $\mathbf{f}_{1:h}$ denotes a portion of token feature $\mathbf{f}$ from the first dimension to the $h$-th dimension. (iii) We compute the new posterior by $\mathcal{P}(\mathbb{N}_{e,i}|\mathbf{f}')=\mathcal{P}(\mathbb{N}_{e,i},\mathbf{f}')/\mathcal{P}^*(\mathbf{f}')$. 

% %we take an additional step to update the posterior probability using the frequency of new data token features through Bayes' theorem. This theorem expresses how the posterior rationally change to account for the availability of related evidence, given by $ P^*({\bf e}|{\bf f})=\frac{P^*({\bf f}|{\bf e})P^*({\bf e})}{P^*({\bf f})}$. Here $P^*(\cdot)$ denotes the profiled probability,
% %$P({\bf e})$ represents the prior probability, $P({\bf f})$ denotes the evidence, and $P({\bf f}|{\bf e})$ denotes the likelihood probability, and $P({\bf e}|{\bf f})$ is the posterior probability. 
% %\begin{equation}\label{By}
% %\small
% %    P({\bf e}|{\bf f})=\frac{P({\bf f}|{\bf e})P({\bf e})}{P({\bf f})},
% %\end{equation}

% \cwu{I do not get what the following is trying to say (if you only have token ID, what are the other dimensions of f?): However, in practice, we only have the unique numerical identifier assigned by a predefined vocabulary (i.e., token ID) as one dimension of the token feature $\mathbf{f}$ to identify a new token. For other dimensions in $\mathbf{f}$, we can obtain marginal probabilities.
% This means we cannot directly use ${\bf f}'$ for a new token and instead the token ID to calculate the adjusted new posterior.}
% Let ${\bf f}'_H$ be the token ID for new data. We rewrite $\mathcal{S}_{k,e,i}({\bf f}')$ in Eq~\ref{ideaby} as $\mathcal{S}_{k,e,i}({\bf f}'_H)$ \cwu{tell the rationale of the following calculation}: %for the Bayesian decision-making policy as:
% \begin{equation}\label{Byderive}
% \small
% \begin{aligned}
%        &\mathcal{S}_{k,e,i}({\bf f}'_H)
%         = \mathcal{P}'({\bf f}'_H)\int_{{\bf f}_{1}}\dots\int_{{\bf f}_{H-1}}\mathcal{P}^*(\mathbb{N}_{e,i}|{\bf f}_{1:H-1},{\bf f}'_H)\\
%         &\frac{\mathcal{P}^*({\bf f}_{1:H-1},{\bf f}'_H)\mathcal{P}'({\bf f}_{1})}{\mathcal{P}^{*}({\bf f}_{2:H-1},{\bf f}'_H)}d{\bf f}_{1}\dots\frac{\mathcal{P}^*({\bf f}_{H-1},{\bf f}'_H)\mathcal{P}'({{\bf f}_{H-1}})}{\mathcal{P}^{*}({\bf f}'_H)}d{\bf f}_{H-1},
% \end{aligned}
% \end{equation}

% \cwu{Rewrite this paragraph to clarify how the above is computed using what data - data from the key-value table and `new data'? The Bayesian decision-making policy is not introduced at all so far so shouldn't be mentioned} The Bayesian decision-making policy with Eq~\ref{Byderive} requires various processing \cwu{what does `various processing' mean?} of profiled data to calculate probabilities. %We first empirically profile token features ${\bf f}$ from at least 100 sampled batches of tokens and their expert selection results in each MoE layer in advance. To manage the profiled data, we create a key-value dataset table, where the primary key consist of token features and expert indices, and the value is the number of tokens satisfying the primary key criteria. 
% Using key search \cwu{what is key search?}, the profiled probabilities in Eq~\ref{Byderive} can be computed by the statistics \cwu{what the statistics are referring to?}. 
%For example, among profiled 10000 tokens, 1000 are with token features ${\bf f}_0$. Expert $0$ at MoE layer $0$ receives 5000 tokens, 200 of which tokens are with ${\bf f}_0$. With the profiles, we establish prior probabilities $P({\bf f}_0)=0.1$ and $P({\bf e}_{0,0})=0.5$, and the likelihood probability $P({\bf f}_0|{\bf e}_{0,0})=0.04$. This allows us to calculate $P({\bf e}_{0,0}|{\bf f}_0)$ for expert selection prediction of new, unprofiled tokens with token feature ${\bf f}_0$.  
%\cwu{tell how much expert selection results are to be profiled/tokens are to be sampled to obtain which probability, prior or likelihood, clearly.}
%However, for new unprofiled tokens, we only have their unique numerical identifier assigned by a predefined vocabulary (i.e. token ID $t_{id}$).
%This means the obtained prior probability  of token features $P(t_{id})$ for new tokens differs from the profiled prior probability $P({\bf f})$, as the token ID $t_{id}$ is only part of the token feature ${\bf f}$. Without $P({\bf f})$, the expert selection $\hat{\bf e}$ cannot be directly obtained from $P({\bf e}|{\bf f})$. Assuming $n$ token features exist in ${\bf n}$, we denote ${\bf f}=\{{\bf f}^1,\dots,{\bf f}^n\}$ and ${\bf f}^n=t_{id}$. Therefore, we use $P({\bf e}|t_{id})$ for expert selection,  %\cwu{explain what $t_{id}$ denotes}.
%\cwu{not clear why this can imply the following} that the expert selection prediction $\hat{\bf e}$ requires the probability $P({\bf e}|t_{id})$ given the token ID $t_{id}$. 
%derived from $P({\bf e}|{\bf f})$ as:

%With Eq.~(\ref{Byderive}), the expert selection $\hat{{\bf e}}$ given the token ID $t_{id}$ can be given by:
%\begin{equation}
%\small
%    \hat{{\bf e}}=\mbox{argmax} P({\bf e}|t_{id}),
%\end{equation}
%where the argmax is over the existing experts at each MoE layer in the MoE model. %\cwu{clarify what the argmax is over}. 
%For example, if a token ID has a $P({\bf e}|t_{id})$ of $\{0.8,0.1,0.05,0.05\}$ for 4 experts at MoE layer $0$, respectively, then this token is routed to the expert $0$ at MoE layer $0$.




\subsection{Scatter-gather communication design}\label{section2B}

%During MoE model inference, all-to-all communication splits and aggregates data in different dimensions before and after the MoE layers. For large data transfers between two serverless functions, the communication needs to traverse the external storage. 
We design pipelined scatter-gather communication at the MoE layer in a serverless platform for better resource utilization and cost reduction. %to minimize the billed cost of all MoE layers with an inference performance guarantee. %\cwu{resource utilization is not the main goal in the paper, but cost minimization and inference performance guarantee}. 


%\cwu{the following is by default what an all-to-all does so not your new design} For scatter, we split the transferred data based on expert selection results from Sec.~\ref{expertselection} to ensure each expert receives only their assigned data.
For a batch of tokens to serve, we set a pipeline degree $\beta$ to split the batch for each expert into minibatches, 
where $\beta$ represents the maximal minibatch size. 
At each MoE layer, the gating network %scatters and 
routes the splitted minibatches to each expert and the next non-MoE layer %receives and 
gathers processed minibatches from each expert.
% \cwu{in the first place, it is never told in the paepr how incoming requests or tokens are batched; then here you only tell about the one all-to-all communication from gating network to experts, what about the data in the other all-to-all communication, from experts to the following operations?}. 
If the minibatch size exceeds the payload limit, indirect transfer through external storage is used; otherwise, direct invocation of the serverless functions is adopted.
%Indirect transfer through the external storage is used if the minibatch size exceeds the limited payload size, and direct invocation of the serverless functions is adopted, otherwise.

Data transfer from the gating network to experts can be pipelined with expert execution based on expert parallelism. Experts do not use pipelining for data transfer to the next non-MoE layer, as this may cause the next non-MoE layer to wait for the execution of experts (e.g., calculation of a minibatch) after receiving the previous processed minibatch. %increasing the running time of non-MoE layers and hence billed cost of the MoE model.
% parallel experts to wait for the execution (e.g. download the processed minibatch of all experts from external storage in turn) in the next non-MoE layer to process the next minibatch before these experts can process the next minibatch, increasing the execution time and billed cost of expert serverless functions. 
% \cwu{there are two all-to-all communications in an MoE layer, one from gating networks to experts and one from experts to the following layer; clarify exactly what you are pipelining each all-to-all communication with}. 
% With pipelining, the download \cwu{download what from where?} and calculation of one minibatch overlap with the upload of \cwu{processing results of?} the previous minibatch to external storage during MoE layers \cwu{what does `during MoE layers' mean?} in a serverless function. %This overlap is possible because the upload processed data is independent of downloading and calculating new data within the function. 
When external storage is involved, with pipelining, the time to download a minibatch from external storage and process this minibatch can overlap with the time to upload the previous processed minibatch to external storage.
% This overlap is only achievable with indirect transfer \cwu{from what to what}, as functions cannot wait for multiple direct data transfers \cwu{wait for multiple direct data transfers for what? not clear how this is related to overlapping download and calculation of one minibatch with the upload of the previous minibatch} while maintaining model parameters in one invocation due to their stateless property.
Note that pipelining is only achievable with indirect transfer via external storage on a serverless platform. Serverless functions are stateless and direct data transfers from other functions require re-invocation of the function each time; model parameters that a serverless function uses are not retained during direct transfers and hence need to be reloaded from external storage for each re-invocation, resulting in significant time and memory waste.
%are invoked after receiving data from direct transfer or an invocation notification message. %\cwu{clarify why These parallelisms enable the overlap, why only overlapping with indirect transfer, the transfer refer to before MoE layer transfer or after MoE layer transfer?}. %between external storage and serverless functions.For simplicity, 
We use one block time to represent the maximal overlap time of the indirect upload of a minibatch and the download and calculation of the next minibatch. 
%one minibatch 
%\cwu{the indirect upload of a minibatch and the download and calculation of the next minibatch?}. %not clear what the maximal overlap time of one minibatch means.
%overlapping the indirect upload of the minibatch and the download and calculation of the next minibatch. 
%The number of block times \cwu{define clearly what a block is} 
The block time is determined by the pipeline degree $\beta$:
%The scatter degree $\beta$ determines the number of blocks, where each block represents the maximum time required to complete overlapped function execution and indirect transfer: 
%\cwu{what the blocks are referring to?}: 
a larger $\beta$ results in fewer minibatches and longer block time. %of one minibatch.  


The benefits of pipelining can be reduced by the access delay to external storage. We design three scatter-gather communication methods tailored for MoE inference on a serverless platform. 
% \cwu{I do not understand the following descriptions and the figures - rewrite explanations and correct the figures (tell each of the cases that the optimization is choosing among clearly):} 
Let $a_e \in\mathbb{A}=\{1, 2, 3\}$ denote three possible scatter-gather communication methods at MoE layer $e$, and we allow all experts at an MoE layer to use the same method to simplify implementation.
Two indirect transfer options exist. 

$\bullet$ In the first option ($a_e=1$), the gating network splits each expert's input into minibatches and sends them to external storage; at each expert, downloading a minibatch from external storage and calculating this minibatch can be overlapped with uploading the previous processed minibatch to external storage. %and then all processed minibatches are downloaded by the next non-MoE layer.
As shown in Fig.~\ref{alltoallfig_indirect}(a), after splitting input data into minibatches of one token each, two minibatches for two experts are stored in external storage (step 1); these two minibatches are downloaded from external storage and calculated by two expert serverless functions, while the next two minibatches are stored in external storage (step 2); the processed minibatches are stored in external storage, while the next two minibatches are downloaded from external storage and calculated by two expert serverless functions (step 3); all processed minibatches are stored in external storage (step 4) and then the next non-MoE layer downloads all minibatches from external storage (step 5). 

$\bullet$ In the second option ($a_e=2$), the gating network transfers each expert's input via external storage to each expert function, and all processed results are downloaded by the next non-MoE layer, without pipelining. As illustrated in Fig.~\ref{alltoallfig_indirect}(b), all input data are stored in external storage (step 1); each expert serverless function downloads its input from external storage (step 2), and stores the processed results in external storage (step 3); then the next non-MoE layer downloads all processed results from external storage (step 4). 

Fig.~\ref{alltoalltimeblockfig_indirect} illustrates the execution time of MoE layers under the two communication designs. %These two options lead to different execution time of MoE layers. %mainly on expert serverless functions. In both Fig.~\ref{alltoalltimeblockfig_indirect}(a) and Fig.~\ref{alltoalltimeblockfig_indirect}(b), 
Stage 1 in both cases represents the time for each expert to start the warm-up function without resource initialization (i.e., short warm start time) and download model parameters, while the gating network concurrently uploads each expert's input to external storage. Stage 2 is the time for each expert to download input from external storage and calculate it, overlapping with the time to start the warm-up function and download model parameters in the next non-MoE layer. In stage 3, the next non-MoE layer downloads the processed results. %of experts' input data in non-MoE layer.

$\bullet$ When using direct transfers ($a_e=3$), the gating network directly transfers each expert's input to the expert serverless function, and the processed results of each expert are directly transferred to the next non-MoE layer, as shown in Fig.~\ref{alltoallfig_direct}. Fig.~\ref{alltoalltimeblockfig_direct} illustrates its execution time. %with direct transfer at the MoE layers.

The total MoE layer time varies with different communication designs. %scatter operation with different scatter degrees, and whether to use pipeline operation. 
We will carefully make the choices in our distributed MoE deployment problem. %to minimize the cost. 


% the scatter-gather communication can either scatter each expert's input data into minibatches and pipeline them to the MoE layers \cwu{what does `pipeline minibatches with MoE layers' mean?} through external storage (i.e, $a_e=1$), as in Fig.~\ref{alltoallfig_indirect}(a), or transfer each expert's input data to the MoE layers through external storage (i.e, $a_e=2$), as in Fig.~\ref{alltoallfig_indirect}(b).   
% These two choices lead to different total execution time at the MoE layers as illustrated in Fig.~\ref{alltoalltimeblockfig_indirect}. Note that in both Fig.~\ref{alltoalltimeblockfig_indirect}(a) and Fig.~\ref{alltoalltimeblockfig_indirect}(b), the latency to start active serverless functions (warm start time) \cwu{no idea what active serverless functions and warm start time mean} and the model download time in MoE execution overlap with the non-MoE execution. MoE layers starts downloading minibatch data only after all data \cwu{what is this `all data' referring to} is stored in external storage to avoid waiting costs for the non-MoE functions. When using direct invocation, the data size at each non-MoE layer can be directly transferred (i.e, $a_e=3$), as shown in Fig.~\ref{alltoallfig_direct}.  Fig.~\ref{alltoalltimeblockfig_direct} illustrates the total execution time with direct transfer at the MoE layers. Note that the total time varies with the different communication approaches, scatter operation with different scatter degrees, and whether to use pipeline operation. %, among which none has an absolute advantage. This leads to a policy-making problem when deploying.
% We will carefully make the choices in our distributed deployment problem, to minimize the cost. 

%Therefore, our designed all-to-all communication can flexibly apply the scatter and pipeline operations to expedite the MoE model inference by setting some parameters. 
 \begin{figure}[!t]
 \centering
 \subfigure[With pipeline operation.]{
   \includegraphics[width=0.4\textwidth]{figs/alltoall_communication.pdf}}
    \centering
 \subfigure[Without pipeline operation.]{
\includegraphics[width=0.4\textwidth]{figs/alltoall_communication1_2.pdf}}
\vspace{-2mm}
 \caption{Scatter-gather communication %in serverless computing
 with indirect transfers through external storage: (a) with pipelining; (b) without pipelining. Pipeline degree $\beta$ is 2.
 }
\label{alltoallfig_indirect}
\vspace{-3mm}
\end{figure}


 \begin{figure}[!t]
 \centering
\includegraphics[width=0.4\textwidth]{figs/alltoall_communication2_2.pdf}
\vspace{-3mm}
 \caption{Scatter-gather communication %in serverless computing 
 with direct function invocation.
 }
\label{alltoallfig_direct}
\vspace{-3mm}
\end{figure}

 \begin{figure}[!t]
 \centering
 \subfigure[With pipeline operation.]{
   \includegraphics[width=0.23\textwidth]{figs/alltoall_communication_time.pdf}}
 \subfigure[Without pipeline operation.]{
   \includegraphics[width=0.23\textwidth]{figs/alltoall_communication_time1_2.pdf}}
   \vspace{-2mm}
 \caption{Scatter-gather communication time %in serverless computing 
 with indirect transfers through external storage: (a) with pipelining; (b) without pipelining.% based on Fig.~\ref{alltoallfig_indirect}.
 }
\label{alltoalltimeblockfig_indirect}
\end{figure}

 \begin{figure}[!t]
 \centering
\includegraphics[width=0.43\textwidth]{figs/alltoall_communication_time2_2.pdf}
\vspace{-3mm}
 \caption{Scatter-gather communication time %in serverless computing 
 with direct function invocation. % based on Fig.~\ref{alltoallfig_direct}.
 }
\label{alltoalltimeblockfig_direct}
\vspace{-5mm}
\end{figure}

\subsection{MoE model deployment% in a serverless computing platform
}\label{Deployformulation}
%For simplicity, we abstract the basic subscript notation using a three tuple $(a_e, e, i)$, where $e\in\mathbb{E}$ denotes MoE layer $e$, $i\in\mathbb{N}_e$ denotes expert $i$ at MoE layer $e$, $a_e \in\mathbb{A}=\{1, 2, 3\},\forall e\in\mathbb{E}$.
%corresponds to three communication methods at MoE layer $e$ with $a_e=1$ for indirect pipelined transfer, $a_e=2$ for indirect unpipelined transfer, and $a_e=3$ for direct transfer. We jointly distribute the MoE model in serverless computing by deciding the communication method (i.e., $a_e$), setting parameters in all-to-all communications (i.e., $\beta$), selecting memory type (i.e., $x_{a_e, e, i}$), and replicating experts (i.e., $y_{a_e, e, i}$). 
%This tuple notation is consistently used throughout this subsection without further explanation. Except for indices and sets, lowercase letters represent unknown variables while uppercase letters represent known values.

The policy maker decides optimal MoE model deployment by making the following decisions:

$\bullet$ Memory size configuration for each serverless function. Let $\mathbb{M}$ be the set of memory size options for each serverless function (e.g., from 128MB to 3008MB on AWS Lambda)
% \cwu{give example memory size options, e.g., on AWS Lambda}). 
%selection decides the computation speed of one serverless function. 
$x_{e,i,j}\in\{0,1\}$ denotes if the $j$-th option in set $\mathbb{M}$ is selected for expert $i$ in MoE layer $e$ %\cwu{for expert i in MoE layer e?} 
(1) or not (0). 
The processing time of one token at expert $i$ in MoE layer $e$, %under all-to-all communication method $a_e$ \cwu{why x and this processing time are related to all-to-all communication method?}, 
% \cwu{clarify the time is from when to when, not that it is not purely just `calculation'; what does E denote in the superscript?}, 
is given by:

\vspace{-5mm}
\begin{equation}
\small
t^{cal}_{e,i}=s_{e,i}\sum^{|\mathbb{M}|}_{j=1}x_{e,i,j}U_j,
        \forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,
\end{equation}
\vspace{-2mm}

\noindent where $s_{e,i}\in\{0,1\}$ denotes if the expert is selected (1) or not (0) for the token (given based on expert selection prediction), %$W_{e,i}$ is the known amount of calculation work (i.e. workload size) in inference for one token \cwu{not clear - does it represent one token's processing time at the expert or the token's size?}, 
and $U_j$ is the time to process one token in an expert
% \cwu{what does unit computation time mean?} 
using the $j$-th memory size option with the serverless function. 

$\bullet$ Expert replication. As the maximal memory size of each serverless function is limited, it is possible that it still takes a long time for a popular expert to process tokens routed to it. Given that an end-to-end inference time target should be met in inference serving, we further consider replicating serverless functions of experts and allow expert replicas to run in parallel for toke processing.
%Expert replication allows the same expert to execute in parallel, reducing the number of tokens handled by each serverless function of the expert. This impacts the choice of communication method.
Let $y_{e,i,g}\in\{0,1\}$ denote if expert $i$ in MoE layer $e$ has $g$ %\cwu{$\mathbb{G}_{e,i,g}$ is a set; g instead?} 
serverless function replicas (1) or not (0), where $g=1, ..., G$ with $G$ as maximal possible replica number
%$\mathbb{G}_{e,i}$ is the replica number option set for the expert (containning consecutive integers starting from 1) \cwu{then you do not need to define $\mathbb{G}_{e,i}$ but just use g=1, ..., G where G is maximal possible replica number}. %to ensure that at least one expert serverless function is available.  
The number of tokens routed to one replica is %given by 
$r_{ e,i}=\sum^{G}_{g=1}y_{e,i,g}d_{e,i}/g$, where $d_{e,i}$ denotes the number of tokens routed to all replicas of the expert.
Let $D^{in}$ be the size of one token and $D^p$ be the maximal payload size in the serverless platform. %\cwu{maximal payload size in the system?}. 
When $r_{e,i} D^{in}>D^p$, direct transfer %should be prohibited 
is not feasible (i.e, ${a_e}=1$ or ${a_e}=2$) at MoE layer $e$. %\cwu{where do you use this, - do you formulate this into any constraint?}.\mf{add to the final constraints}

$\bullet$ Scatter-gather communication method and parameter ($\beta$). We seek to minimize the total billed cost of all MoE layers. 
% The billed cost of gating network can be ignored here as it affect the billed cost of all MoE layers little 
% the memory configuration of serverless functions of the gating networks does not depend on expert popularity and \cwu{not clear what point the following sentence is trying to make} the impact of scatter-gather communication methods on \cwu{whose?} execution time is also reflected in the experts. 
The billed cost of the gating network can be ignored here, as it affects the cost of all MoE layers little: the memory size of serverless functions for gating networks does not depend on expert popularity, and the impact of scatter-gather communication methods on the gating network's execution time is also reflected in the experts.
Hence, we consider the total billed cost of all MoE layers to be the billed cost of all experts in MoE layers. 
The billed cost of MoE layer $e$ is then given by $c_e=(a_e-2)(a_e-3)c_{1,e}+(a_e-1)(a_e-3)c_{2,e}+(a_e-1)(a_e-2)c_{3,e}$, where the billed cost of MoE layer $e$ under the communication method $a_e$ is: % expressed as:
\vspace{-1mm}
\begin{equation}
    \small
    c_{a_e,e}=\sum_{i\in \mathbb{N}_e}s_{e,i}t_{a_e,e,i}\sum^M_{j=1}x_{e,i,j}\mathbb{M}_j,\forall e\in\mathbb{E},\forall a_e\in\mathbb{A},
\end{equation}
Here $\mathbb{M}_j$ represents the $j$-th memory size in set $\mathbb{M}$, and %\cwu{what is $\mathbb{M}_j$?}
$t_{a_e,e,i}$ is the total execution time of all replicas of the expert:
\vspace{-1mm}
\begin{equation}
    \small
t_{a_e,e,i}=\sum^{G}_{g=1}y_{e,i,g} g t^{rep}_{a_e,e,i},\forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\forall a_e\in\mathbb{A},\label{firstconst}
\end{equation}
where $t^{rep}_{a_e,e,i}$ denotes the execution time of one replica of the expert. 
$t^{rep}_{a_e,e,i}$ is related to the scatter-gather communication method chosen. %We discuss three cases in obtaining $t^{rep}_{a_e,e,i}$. %: $a_e=1$, $a_e=2$ and $a_e=3$.
We give formulars of three cases in obtaining $t^{rep}_{a_e,e,i}$.

\vspace{1mm}
\noindent\textit{(1) Pipelined indirect transfer %}: For pipelined indirect transfer (i.e., 
($a_e=1$).} %Assuming each block contains at most $\beta$ tokens as a minibatch per expert and represents the maximum time for the overlapped upload of one minibatch and the download and calculation of another minibatch, 
We have %The execution time $t^{rep}_{1,e,i}$ of one replica of the expert is given by: %Eq~\ref{eq_t1rep}:
% \iffalse
% \begin{subequations}
%     \small
%     \begin{align}
%     &t^{rep}_{1,e,i}=T^{h,E}_{e,i}+t^{nblk}_{1,e,i}+n_{1,e,i}t^{blk}_{1,e,i},\forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{eq_t1rep}\allowdisplaybreaks\\
%     &t^{nblk}_{1,e,i}=2T^{dl}+\beta(\frac{D^{in}+D^{o}}{B^s}+t^{cal,E}_{1,e,i}),
%         \forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{eq_nblk}\allowdisplaybreaks\\  
%     &n_{1,e,i}=\lceil\frac{r_{1,e,i}}{\beta}\rceil-1,\forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{eq_n}\allowdisplaybreaks\\
%      &t^{blk}_{1,e,i}=T^{dl}+\beta\max\{\frac{D^{in}}{B^s}+t^{cal,E}_{1,e,i},\frac{D^{o}}{B^s}\},
%         \forall e\in \mathbb{E},\forall i \in \mathbb{N}_e, \label{Eq_blk}
%     \end{align}
% \end{subequations}
% where, for all replicas of the expert, $n_{1,e,i}$ in Eq~\ref{eq_n} is the number of all overlapped block in one replica; the known head time $T^{h,E}_{e,i}=\frac{P_{e,i}}{B^s}+T^{dl}+T^{str}$ consists of the warm start time $T^{str}$, the access delay to external storage $T^{dl}$ and the model download time $\frac{P_{e,i}}{B^s}+T^{dl}$ with the bandwidth $B^s$ between external storage and serverless function and the parameter size $P_{e,i}$ of the expert; the non-block time $t^{nblk}_{1,e,i}$ in Eq~\ref{eq_nblk} excludes the blocks time or head time; and $t^{blk}_{1,e,i}$ in Eq~\ref{Eq_blk} denotes the worst-case execution time of one block, where the term $\max\{\frac{D^{in}}{B^s}+t^{cal,E}_{1,e,i},\frac{D^{o}}{B^s}\}$ represents the maximal time of the  overlapped upload of one token and the download and calculation of another token.
% \fi
\begin{equation}
    \small
t^{rep}_{1,e,i}=T^{h,E}_{e,i}+t^{nblk}_{e,i}+\beta t^{blk}_{e,i},\forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{eq_t1rep}
\end{equation}
where %$n_{e,i}=\lceil\frac{r_{e,i}}{\beta}\rceil$ is the number of all blocks (\cwu{still not clear if `a block' is a time concept or a minibatch size concept}each overlaps downloading a minibatch from external storage and calculating this minibatch with uploading the previous processed minibatch to external storage) in one replica \cwu{how to understand `blocks in one replica'?}.  
the head time $T^{h,E}_{e,i}=\frac{P_{e,i}}{B^s}+T^{dl}+T^{str}$ consists of warm start time $T^{str}$, the access delay to external storage $T^{dl}$ and the model download time $\frac{P_{e,i}}{B^s}+T^{dl}$ with bandwidth $B^s$ between external storage and serverless function and the parameter size $P_{e,i}$ of the expert. %The time \cwu{how to understand `non-block' time?}
$t^{nblk}_{e,i}=T^{dl}+\lceil\frac{r_{e,i}}{\beta}\rceil(\frac{D^{o}}{B^s})$ includes the time to upload the last minibatch to external storage %\cwu{what does `in external' mean?} 
and $D^{o}$ is the size of the processed result of one token by an expert. 
$t^{blk}_{1,e,i}=T^{dl}+\beta\max\{\frac{D^{in}}{B^s}+t^{cal}_{e,i},\frac{D^{o}}{B^s}\}$ denotes one worst-case block time. 
%where the term $\max\{\frac{D^{in}}{B^s}+t^{cal}_{e,i},\frac{D^{o}}{B^s}\}$ represents the maximal time of the overlapped upload of one token and the download and calculation of another token. %Overall, the execution time of one replica of an expert consists of the head time in stage 1, and the time to execute all blocks and the non-block time in stage 2, at the row of an expert in Fig.~\ref{alltoalltimeblockfig_indirect}(a).
%\cwu{explain in high level what the execution time one replica of the expert includes and point to earlier figure that may have illustrate the time composition.} 


The latency, %\cwu{rewrite what this latency is from when to when, or include what time composition}
% from the calculation and data sending of the previous non-MoE layer \cwu{this is not one time point}, through the MoE layer $e$, to the model download and data receiving of the next non-MoE layer
from the earlist time point when expert serverless functions start or the gating network starts to transfer each expert's input, to the latest time when the next non-MoE layer finishes downloading the processed results of all experts from external storage or finishes downloading model parameters with direct transfer, is referred to as MoE-E2E latency %. The MoE-E2E latency 
$t^{lat}_{1,e}$: % is given by: %Eq~\ref{eq_tlat1}:
% \iffalse
% \begin{subequations}
%     \small
%     \begin{align}
%       &t^{lat}_{1,e}=\max\{t^{S1}_{1,e}+t^{S234}_{1,e},T^{load}_e\}+t^{h,NE}_{1,e},\forall e\in \mathbb{E},\label{eq_tlat1}\allowdisplaybreaks\\ 
%       &t^{S1}_{1,e}=\max_{i\in\mathbb{N}_e}\{T^{h,E}_{e,i},t^{t,NE}_{1,e}\},\forall e\in \mathbb{E},\label{eq_ts11}\allowdisplaybreaks\\
%       &t^{t,NE}_{1,e}=T^{cal,NE}_e+T^{dl}+\frac{\beta D^{o}}{B^s},\forall e\in \mathbb{E},\label{eq_ttne1}\allowdisplaybreaks\\
%       &t^{S234}_{1,e}=\max_{i\in\mathbb{N}_e}\{t^{rep}_{1,e,i}-T^{h,E}_{e,i}\},\forall e\in \mathbb{E},\label{eq_ts234}\allowdisplaybreaks\\
%       &t^{h,NE}_{1,e}=\sum_{i \in \mathbb{N}_e}\sum^{|\mathbb{G}_{e,i}|}_{g=1}y_{1,e,i,g}\mathbb{G}_{e,i,g}\nonumber\\&\qquad\qquad\qquad((n_{1,e,i}+1)T^{dl}+\frac{r_{1,e,i}D^{in}}{B^s}),\forall e\in \mathbb{E},\label{eq_thne1}
%     \end{align}
% \end{subequations}
% where, as shown in Fig.~\ref{alltoalltimeblockfig_indirect}(a), $t^{S1}_{1,e}$ in Eq~\ref{eq_ts11} represents the time of the $S1$ stage, and $t^{S234}_{1,e}$ in Eq~\ref{eq_ts234} denotes the time from $S2$ to $S4$ stages. The tail time of the previous non-MoE layer $t^{t,NE}_{1,e}$ in Eq~\ref{eq_ttne1} consists of the calculation time $T^{cal,NE}_e$ and data sending time $T^{dl}+\frac{\beta D^{o}}{B^s}$. For the next non-MoE layer, the head time $T^{lead}_e$ includes the warm start time and the download model time, and $t^{h,NE}_{1,e}$ in Eq~\ref{eq_thne1} denotes the data receiving time. The term $\max\{t^{S1}_{1,e}+t^{S1234}_{1,e},T^{load}_e\}$ denotes the time from the $S1$ to $S4$.
% %\cwu{why adding the number of blocks in time computation?}. 
% \fi
\begin{equation}
    \small
      t^{lat}_{1,e}=\max\{t^{S12}_{1,e},T^{load}_e\}+t^{S3}_{1,e},\forall e\in \mathbb{E},\label{eq_tlat1}
\end{equation}
where %, as shown in Fig.~\ref{alltoalltimeblockfig_indirect}(a), $t^{S12}_{1,e}=\max_{i\in\mathbb{N}_e}\{T^{h,E}_{e,i},\lceil\frac{r_{e,i}}{\beta}\rceil\frac{D^o}{B^s}\}+t^{nblk}_{e,i}+n_{e,i}t^{blk}_{e,i}$ represents the time to start the expert serverless function and download model parameters from external storage, while a minibatch is concurrently being uploaded to external storage (stage 1), and the time to download minibatches from external storage, calculate these minibatches, and upload the processed minibatches to external storage (stage 2). $t^{S3}_{1,e}=n_{e,i}(T^{dl}+\lceil\frac{r_{e,i}}{\beta}\rceil\frac{ D^{in}}{B^s})$ denotes the time to download the processed results of all experts%' input data
%from external storage (stage 3). %\cwu{tell what the $S1$, $S2$ to $S4$ stages are for}. 
%The tail time of the previous non-MoE layer $t^{t,NE}_{1,e}=T^{cal,NE}_e+T^{dl}+\frac{\beta D^{o}}{B^s}$ consists of the calculation time $T^{cal,NE}_e$ and data sending time $T^{dl}+\frac{\beta D^{o}}{B^s}$ \cwu{data sending to what}. 
$T^{load}_e$ includes the time to start the serverless function of non-MoE layer and download the model parameters. 

These formulars are derived based on Fig.~\ref{alltoalltimeblockfig_indirect}(a) and details omitted due to space limit.
%, and $t^{h,NE}_{1,e}=\sum_{i \in \mathbb{N}_e}\sum^{|\mathbb{G}_{e,i}|}_{g=1}y_{1,e,i,g}g((n_{1,e,i}+1)T^{dl}+\frac{r_{1,e,i}D^{in}}{B^s})$ denotes the data receiving time. The term $\max\{t^{S1}_{1,e}+t^{S1234}_{1,e},T^{load}_e\}$ denotes the time from $S1$ to $S4$.
%\cwu{why adding the number of blocks in time computation?}. 

\vspace{1mm}
\noindent\textit{(2) Non-pipelined indirect transfer ($a_e=2$).} We have %For unpipelined indirect transfer (i.e., $a_e=2$), 
%The execution time $t^{rep}_{2,e,i}$ of one replica of the expert is : %given by Eq~\ref{Eq_rep2}:
% \iffalse
% \begin{subequations}
%     \small
%     \begin{align}
% &t^{rep}_{2,e,i}=T^{h,E}_{e,i}+2T^{dl}+t^{data}_{2,e,i},
% \forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{Eq_rep2}\\
% &t^{data}_{2,e,i}=r_{2,e,i}(\frac{D^{in}+D^{o}}{B^s}+t^{cal,E}_{2,e,i}),
% \forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{eq_data2}
%     \end{align}
% \end{subequations}
% where $t^{data}_{2,e,i}$ in Eq~\ref{eq_data2} denotes the data receiving, calculation, and sending time in one replica of the expert. 
% %\cwu{how the terms are calculated should be briefly explained}:
% \fi
\begin{equation}
    \small
t^{rep}_{2,e,i}=T^{h,E}_{e,i}+2T^{dl}+t^{data}_{2,e,i},
\forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,\label{Eq_rep2}
\end{equation}
where $t^{data}_{2,e,i}=r_{e,i}(\frac{D^{in}+D^{o}}{B^s}+t^{cal}_{e,i})$.  %denotes the time to download the replica's input from external storage, calculate the input, and upload the processed results to external storage by one replica of the expert. 
%\cwu{how the terms are calculated should be briefly explained}:

The MoE-E2E latency is: %$t^{lat}_{2,e}$ can be given by Eq~\ref{eq_lat2}:
% \iffalse
% \begin{subequations}
%     \small
%     \begin{align}
%        &t^{lat}_{2,e}=\max\{t^{S1}_{2,e}+t^{S23}_{2,e},T^{load}_e\}+t^{h,NE}_{2,e},\forall e\in \mathbb{E}, \label{eq_lat2}\allowdisplaybreaks\\
%        &t^{S1}_{2,e}=\max_{i\in\mathbb{N}_e}\{T^{h,E}_{e,i},t^{t,NE}_{2,e}\},\forall e\in \mathbb{E},\label{eq_s12}\allowdisplaybreaks\\
%        &t^{t,NE}_{2,e}=T^{cal,NE}_e+ T^{dl}+\frac{\max_{i\in\mathbb{N}_e}\{r_{2,e,i}\} D^{o}}{B^s},\forall e\in \mathbb{E},\label{eq_ttne2}\allowdisplaybreaks\\
%        &t^{S23}_{2,e}=\max_{i\in\mathbb{N}_e}\{t^{rep}_{2,e,i}-T^{h,E}_{e,i}\},\forall e\in \mathbb{E},\label{eq_s23}\allowdisplaybreaks\\
%        &t^{h,NE}_{2,e}=\sum_{i \in \mathbb{N}_e}\sum^{|\mathbb{G}_{e,i}|}_{g=1}y_{2,e,i,g}\mathbb{G}_{e,i,g}(T^{dl}+\frac{r_{2,e,i}D^{in}}{B^s}),\forall e\in \mathbb{E},\label{eq_thne2}
%     \end{align}
% \end{subequations}
% where, as shown in Fig.~\ref{alltoalltimeblockfig_indirect}(b), $t^{S1}_{2,e}$ in Eq~\ref{eq_s12} represents the time of the $S1$ stage, and $t^{S23}_{2,e}$ in Eq~\ref{eq_s23} denotes the time from $S2$ to $S3$ stages. The tail time of the previous non-MoE layer $t^{t,NE}_{2,e}$ in Eq~\ref{eq_ttne2} consists of the calculation and data sending time. $t^{h,NE}_{2,e}$ in Eq~\ref{eq_thne2} denotes the data receiving time for the next non-MoE layer.
% \fi
\begin{equation}
    \small
       t^{lat}_{2,e}=\max\{t^{S12}_{2,e},T^{load}_e\}+t^{S3}_{2,e},\forall e\in \mathbb{E}. \label{eq_lat2}
\end{equation}
%where, as shown in Fig.~\ref{alltoalltimeblockfig_indirect}(b), $t^{S12}_{2,e}=\max_{i\in\mathbb{N}_e}\{T^{h,E}_{e,i},t^{data}_{2,e,i}\}$ represents %the time to start the expert serverless function and download model parameters from external storage while each replica's input is concurrently uploaded to external storage (stage 1) and the time to download the replica's input from external storage, calculate the input data, and upload the processed results of all experts to external storage (stage 2). 
%the stage 1 and stage 2 time, and $t^{S3}_{2,e}=T^{dl}+\frac{r_{e,i}D^{in}}{B^s}$ is the stage 3 time. %time to download the processed results of all experts from external storage (stage 3).
% and $t^{S23}_{2,e}=\max_{i\in\mathbb{N}_e}\{t^{rep}_{2,e,i}-T^{h,E}_{e,i}\}$ denotes the time from $S2$ to $S3$ stages \cwu{tell what the stages do}. The tail time of the previous non-MoE layer $t^{t,NE}_{2,e}=T^{cal,NE}_e+ T^{dl}+\frac{\max_{i\in\mathbb{N}_e}\{r_{2,e,i}\} D^{o}}{B^s}$ consists of the calculation and data sending time. $t^{h,NE}_{2,e}=\sum_{i \in \mathbb{N}_e}\sum^{|\mathbb{G}_{e,i}|}_{g=1}y_{2,e,i,g}g(T^{dl}+\frac{r_{2,e,i}D^{in}}{B^s})$ denotes the data receiving time for the next non-MoE layer.

These formulars are derived based on Fig.~\ref{alltoalltimeblockfig_indirect}(b) and details omitted due to space limit

\vspace{1mm}
\noindent \textit{(3) Direct transfer ($a_e=3$).} We have: %The execution time $t^{rep}_{3,e,i}$ of one replica of the expert is: % given by Eq~\ref{eq_rep3}:
\vspace{-1mm}
\begin{equation}\label{eq_rep3}
    \small
        t^{rep}_{3,e,i}=T^{h,E}_{e,i}+r_{e,i}(\frac{D^{o}}{B^f}+t^{cal}_{e,i}),\forall e\in \mathbb{E},\forall i \in \mathbb{N}_e,
        \vspace{-1mm}
\end{equation}
where $B^f$ is the bandwidth between serverless functions.

The MoE-E2E latency $t^{lat}_{3,e}$ is: % given by Eq~\ref{eq_lat3}:
% \iffalse
% \begin{subequations}
%     \small
%     \begin{align}
%         &t^{lat}_{3,e}=\max_{ i \in \mathbb{N}_e}\{t^{rep}_{3,e,i}\}+t^{t,NE}_{3,e}+T^{load}_e,\forall e\in \mathbb{E},\label{eq_lat3}\\
%     &t^{t,NE}_{3,e}=T^{cal,NE}_e+\frac{\max_{i \in \mathbb{N}_e}\{r_{3,e,i}\}D^{o}}{B^f},\forall e\in \mathbb{E},\label{lasteq}
%     \end{align}
% \end{subequations}
% where the tail time of the previous non-MoE layer $t^{t,NE}_{3,e}$ in Eq~\ref{lasteq} consists of the calculation and direct transfer time.
% \fi
\vspace{-1mm}
\begin{equation}
    \small
        t^{lat}_{3,e}=\frac{r_{e,i}D^{in}}{B^f}+\max_{ i \in \mathbb{N}_e}\{t^{rep}_{3,e,i}\}+T^{load}_e,\forall e\in \mathbb{E}.\label{eq_lat3}
        \vspace{-1mm}
\end{equation}
% where the tail time of the previous non-MoE layer $t^{t,NE}_{3,e}=T^{cal,NE}_e+\frac{\max_{i \in \mathbb{N}_e}\{r_{3,e,i}\}D^{o}}{B^f}$ consists of the calculation and direct transfer time.

The MoE-E2E latency at MoE layer $e$ is given by $t^{lat}_{e}=(a_e-2)(a_e-3)t^{lat}_{1,e}+(a_e-1)(a_e-3)t^{lat}_{2,e}+(a_e-1)(a_e-2)t^{lat}_{3,e}$.

%The variable $x$ of memory size configuration and the variable $y$ of expert replication affect the execution time of a replica of an expert and MoE-E2E latency, which are obtained in different ways under different method $a_e$. This may result in different communication methods being optimal for the varying values of $x$ and $y$. Hence, the choices of $a_e$ is implicitly captured in decision variables x and y in our cost minimization problem. \cwu{but I thought your definition of $c_e$ now includes variable $a_e$ explicitly}.


%Hence, the billed cost $c^{a_e}_{e}$ of all experts at the MoE layer $e$ under the communication method $a_e$ can be given by:
%\begin{equation}
%\small
%    c^{a_e}_{e}=\sum_{i\in \mathcal{N}_e}s_{e,i}T^{a_e}_{e,i}\sum^M_{j=1}x_{a_e,e,i,j}M_j,\forall e\in\mathcal{E}.
%\end{equation}

%Similarly, the end-to-end inference time $T$ of the MoE model 
%in the inference with one batch of input request 
%\cwu{clarify what one inference execution is} 
%is:
%\begin{equation}\label{eqtotal_time}
%\small
%    T=T^{head}+T^{tail}+\sum_{e\in \mathcal{E}}T^{a_e}_{e},
%\end{equation}
%where $T^{head}$ is the execution time of the first non-MoE layer without calculation and data transfer time, %\cwu{clarify what the task head is},
%and $T^{tail}$ denotes the execution time of the last non-MoE layer without model download and data receiving time.







%Therefore, based on the expert prediction results, 
\noindent\textbf{Optimal MoE deployment problem:} We formulate optimal deployment of MoE model inference in a serverless platform to minimize the billed cost of all MoE layers (i.e., $\sum_{e\in\mathbb{E}}c_{e}$), by jointly deciding the communication method (i.e., $a_e$), selecting memory size configurations (i.e. $x_{e,i})$, deciding expert replication (i.e. $y_{e,i}$), and setting parameter $\beta$ for pipelined scatter-gather communication.

\begin{subequations}\label{formulation_v1}
\small
  \begin{align}
  &\min\sum_{e\in\mathbb{E}}c_{e} \label{obj}\\
     &\text{subject to }\quad\ref{firstconst}-\ref{eq_lat3} \label{formulation_v1_b},\\
&P_{e,i}+M^{itrm}_{e,i}+r_{e,i}(D^{in}+D^{o})\nonumber\\
&\qquad \leq\sum^{|\mathbb{M}|}_{j=1}x_{e,i,j}\mathbb{M}_j, \forall e \in \mathbb{E},\forall i\in \mathbb{N}_e\allowdisplaybreaks\label{memory_limit}\\
&T^{head}+T^{tail}+\sum_{e\in \mathbb{E}}(t^{lat}_{e}+T^{NE}_e)\leq T^{limit},\label{time_limit}\\
&1\leq\beta\leq \max_{i\in \mathbb{N}_e, e\in \mathbb{E}}r_{e,i},\allowdisplaybreaks\label{beta_limit}\\
&(a_e-3)(r_{e,i}D^{in}-D^p)\leq 0,\forall e\in \mathbb{E},\forall i\in \mathbb{N}_e,\forall a_e\in\mathbb{A}, \allowdisplaybreaks\label{direct_limit}\\
&\sum^{|\mathbb{M}|}_{j=1}x_{e,i,j}=1,\forall e\in \mathbb{E},\forall i\in \mathbb{N}_e,\allowdisplaybreaks\\
&\sum^{G}_{g=1}y_{e,i,g}=1,\forall e\in \mathbb{E},\forall i\in \mathbb{N}_e,\allowdisplaybreaks\\
&x_{e,i,j}\in\{0,1\}, \forall e \in \mathbb{E},\forall i\in \mathbb{N}_e,\forall j \in \mathbb{M},\allowdisplaybreaks\\
&y_{e,i,g}\in\{0,1\},\forall e \in \mathbb{E},\forall i\in \mathbb{N}_e,  \forall g \in \mathbb{G}_{e,i},\allowdisplaybreaks\\
&\beta\in \mathbb{Z},
  \end{align}
\end{subequations}
Here $M^{itrm}_{e,i}$ is the memory size of intermediate results during an expert's inference.  
$T^{limit}$ is the time limit of end-to-end MoE model inference (i.e., serving SLO). %and typically set as the time to generate the results of all inference request at human level reading speed; 
$T^{head}$ is the execution time of the serverless function of the first non-MoE layer. %and the subsequent gating network without the time to transfer each input's data to experts; %\cwu{how is this $T^{head}$ related to earlier time formulations?},
$T^{tail}$ is the execution time of the serverless function of the last non-MoE layer, excluding the time to receive data from the last MoE layer or download them from external storage. %the processed results of all experts' input data, and 
$T^{NE}_e$ is the processing time %to calculate inference requests in the serverless function 
of non-MoE layer $e$ with the subsequent gating network. %\cwu{how is this $T^{tail}$ related to earlier time formulations?}. 
(\ref{memory_limit}) specifies the memory limit of each serverless function, (\ref{time_limit}) gives the end-to-end inference time target of the MoE model,
(\ref{beta_limit}) limits the maximal number of tokens in each block in calculating the worst-case total time, and (\ref{direct_limit}) prohibits direct tranfers when the payload size is below transferred data size between the gating network and each expert, as well as between each expert and the next non-MoE layer.





==> Sec4-Algorithm.tex <==
\section{The BO Framework}\label{secAlg}
We now present our BO algorithm for the BO framework to learn expert selection predictions and optimize MoE model deployment, together with an efficient algorithm to solve the optimal MoE model deployment by the policy maker. % the billed cost of all MoE layers in serverless computing. We start with policy maker design with the ODS algorithm, assuming expert selection results are given; then we devise the BO algorithm to control our entire system, which includes a feedback processor to fine-tune expert selection predictions. This algorithm works with the policy maker to minimize the billed cost.

\subsection{Optimal MoE Deployment Algorithm}
%\textbf{Policy maker:} 
Given expert selection results, the optimal MoE deployment problem in (\ref{formulation_v1}) %\ref{obj}
is a MIQCP problem with a non-linear objective in (\ref{obj}), quadratical constraints in  (\ref{memory_limit}) and (\ref{direct_limit}), binary variables $x$ and $y$, and integer variable $\beta$ and $a$. MIQCP problems are in general NP-hard \cite{elloumi2019global} because of their non-linearity and %the presence of 
discretized variables. % prevent them from being solved in polynomial time.
% \cwu{mixed-integer quadratically constrained programming (MIQCP) problem 
% \cwu{why it is mixed-integer and quadratically constraine?}}. 
%\cwu{Explain why it is NP-hard problem}. 
We design an efficient algorithm to solve it approximately. 

We first divide problem~(\ref{formulation_v1}) into three cases by fixing the scatter-gather communication method: $a_e=1$,$\forall e\in\mathbb{E}$; $a_e=2$,$\forall e\in\mathbb{E}$; and $a_e=3$,$\forall e\in\mathbb{E}$. We then linearize max functions in (\ref{obj}), (\ref{time_limit}) and (\ref{beta_limit}) %\cwu{point to max functions in which constraints} 
by adding auxilliary variables  
%when $x \in \mathbb{X}$ is a continuous variable, 
($\max_{h\in \mathbb{H}}\{h\}$ can be
linearized as $\phi\geq h$, $\forall h \in \mathbb{H}$%\cwu{f and x have been used to denote other meanings in paper - change the symbols}
). 
Then we solve each resulting MIQCP by a solver \cite{Gurobi}, respectively, and obtain costs $c_{1,e}$, $\forall e\in\mathbb{E}$, $c_{2,e}$, $\forall e\in\mathbb{E}$, and $c_{3,e}$, $\forall e\in\mathbb{E}$, from the three solutions. %We assume that at least one solution exist within three MIQCPs and 
%We set $c_{a',e}=\infty$, $\forall e\in\mathbb{E}$, if no solution is obtained for the respective MIQCP. %at $a=a'$. 
Based on these solutions, we design an Optimal Deployment Selection (ODS) algorithm to decide $a_e$ for each MoE layer, as given in Alg~\ref{alg_optimal_deploy}. 

For each MoE layer $e$, we select the communication method $\hat{a}_e$ with the lowest cost, set all experts to use the same method, %\cwu{what is the rationale behind - why choosing the smallest cost computed by setting all MoE layers to use the same communication method, for one MoE layer?} 
and then calculate the MoE-E2E latency $\hat{t}^{lat}_{\hat{a}_e,e}$ (lines 4-7). If the new MoE-E2E latency satisfies the end-to-end inference time constraint, the optimal deployment policy for the MoE model is obtained; otherwise, we identify the MoE layer $\tilde{e}$ with the highest latency, set the cost of the corresponding scatter-gather communication $\tilde{a}_{\tilde{e}}$ to infinity (lines 10-12), and then iteratively decide $\hat{a}_e$ for each MoE layer (lines 3-17). At most $2|\mathbb{E}|$ iterations are needed, as three communication methods provide up to $3|\mathbb{E}|$ solutions of $\hat{a}_e$, $\forall e\in\mathbb{E}$, and selecting $|\mathbb{E}|$ solutions excludes up to $2|\mathbb{E}|$ other solutions.
%\cwu{clarify why doing at most $2|\mathbb{E}|$ iterations}.
%Here the memory constraint is not considered as it is already satisfied in the solution by the MIQCP solver. 
If all costs $c_{a_e,e}$ become infinity, %while no feasible solution exists, 
it implies that mixing different communication methods across different MoE layers do not work. In this case, we return the optimal deployment policy with the lowest cost with all MoE layers using the same scatter-gather communication method (lines 18-20).

\subsection{BO algorithm} 


%\cwu{what is the objective in practical problems?}. 
 % \cwu{clarify what the raw data means and what associate with expert selection results means}, 
%\cwu{is new data pattern generation related to billed cost? why need to generate it after obtaining the cost?}. 

\begin{algorithm}[!t]
\small
   \caption{Optimal Deployment Selection Algorithm of an MoE model (ODS) %\cwu{the algorithm should specify both input and output}
   }
    \label{alg_optimal_deploy}
    \begin{algorithmic}[1]
    
        \REQUIRE Optimal solutions $x_{a,e,i}$, $y_{a,e,i}$, $\beta$ and optimal objective $c_{a,e}$,$\forall e\in\mathbb{E}$,$\forall i\in\mathbb{N}_e$ of solving three MIQCP problems with fixed $a$,$\forall a \in \mathbb{A}$
        %\cwu{clarify if they are the solutions of solving the three MIQCP problem with fixed $a_e$} %and $c_{a,e}\neq$ infinity,$\forall e\in\mathbb{E}$, $\exists a\in \mathbb{A}$.
        \ENSURE $\hat{a}_e$, $\beta$, $x_{\hat{a}_e,e,i}$,$y_{\hat{a}_e,e,i}$,$\forall e\in\mathbb{E}$,$\forall i\in\mathbb{N}_e$%Selected scatter-gather communication method $\hat{a}_e$ and parameter $\beta$, memory configuration variable $x_{\hat{a}_e,e,i}$, and expert replication $y_{\hat{a}_e,e,i}$,$\forall e\in\mathbb{E}$,$\forall i\in\mathbb{N}_e$
        % \STATE $c_e=[c_{1,e},c_{2,e},c_{3,e}]$ with $\forall e\in\mathbb{E}$.
        \STATE itr=0.
        \WHILE{%True and 
        itr$\leq2|\mathbb{E}|$}
        \FOR{$e\in\mathbb{E}$ %\cwu{why R}?
        }
        \FOR{$i\in\mathbb{N}_e$}
        \STATE $\hat{a}_e=argmin_{a_e\in\mathbb{A}}[c_{1,e},c_{2,e},c_{3,e}]$; %\cwu{$c_e$ is a set; can you do argmin on a set?}.
        \STATE Calculate the MoE-E2E latency $\hat{t}^{lat}_{\hat{a}_e,e}$.
        \ENDFOR
        \ENDFOR
        \IF{$T^{head}+T^{tail}+\sum_{e\in\mathbb{E}}(\hat{t}^{lat}_{\hat{a}_e,e}+T^{NE}_e)>T^{limit}$}
        \STATE $\tilde{a}_{\tilde{e}},\tilde{e}=argmin_{e\in\mathbb{E}}\hat{t}^{lat}_{\hat{a}_e,e}$;
        \STATE Set $c_{\tilde{a}_{\tilde{e}},\tilde{e}}=\infty$.
        \ELSE \RETURN $\hat{a}_e$, $x_{\hat{a}_e,e,i}$, $y_{\hat{a}_e,e,i}$, $\beta$,$\forall e\in\mathbb{E}$,$\forall i\in\mathbb{N}_e$.
        \ENDIF
        \STATE itr+=1.
        \ENDWHILE
        \IF{itr$>2|\mathbb{E}|$}
        \STATE $\hat{a}=argmin_{a\in\mathbb{A}}\sum_{e\in\mathbb{E}}c_{a,e}$
        \RETURN $\hat{a}$, $x_{\hat{a},e,i}$, $y_{\hat{a},e,i}$, $\beta$,$\forall e\in\mathbb{E}$,$\forall i\in\mathbb{N}_e$.
        \ENDIF
    \end{algorithmic}
\end{algorithm}



\begin{algorithm}[!th]
\small
   \caption{Bayesian Optimization Algorithm with Multiple-dimension ${\bf \epsilon}$-Greedy Search %\cwu{both input and output of the algorithm should be specified}
   }
    \label{alg1}
    \begin{algorithmic}[1]
        \REQUIRE MoE model, dataset table $\Omega_0$, %\cwu{D has been used for other meaning like in $D^0$ - change the symbol},
        normal range of key-value pairs $\mathbb{P}$,%\cwu{inconsistent with that in text} as $\mathbb{P}$ without token IDs' range \cwu{inconsistent with that in text}, 
        and constants $Q$, $\mu$, $\alpha$, $\rho$, $\rho_1$, $\rho_2$, $\rho_3$, $\lambda$, $\zeta$.
        \ENSURE optimal key-value pairs $\{\hat{{\bf z}}_{q},\hat{v}_{q}\}_{q\in\{1,\dots,Q\}}$
        \STATE Initialize Q key-value pairs $\{{\bf z}_{0,q}, v_{0,q}\}_{\forall q \in\{1,\dots,Q\}}$ for key-value table, ${\bf \epsilon}_0\in\mathbb{R}^{Q}$ for ${\bf \epsilon}$-GS, limited range of key-value pairs $\mathbb{L}$, BO historical set %\cwu{is `BO params-value set' a commonly used term?}
        $\mathbb{B}_0=\{\}$, and the BO trial index $\tau=1$.
        \REPEAT%{$\tau=1,\dots,\Lambda$ \cwu{why specify T BO iterations instead of using other optimality termination criteria? Note T has been used earlier and the symbol needs change}}
        \STATE ${\bf \epsilon}_{\tau}=\frac{{\bf \epsilon}_0}{1+\rho \tau}$.
        \STATE $\Omega_\tau({\bf z}_{\tau-1,q})=v_{\tau-1,q}$,$\forall q \in\{1,\dots,Q\}$.
        \STATE $\hat{i}_{e}=argmax_{i\in\mathbb{N}_e} \mathcal{P}(\mathbb{N}_{e,i}|{\bf f}'_1)$,$\forall e \in \mathbb{E}$ with $\Omega_{\tau}$.
        \STATE $c_{\tau,a,e}$ from three MIQCP solvers,$\forall e\in\mathbb{E},\forall a\in\mathbb{A}$.
        \STATE $(\hat{a}_e, x_{\hat{a}_e,e,i},y_{\hat{a}_e,e,i},\beta)_{\tau}$=ODS($c_{\tau,a,e}$),$\forall a\in\mathbb{A}$, $\forall e\in\mathbb{E}$, $\forall i\in\mathbb{N}_e$.
        \FOR{$j=1,\dots,J$}
        \FOR{$e\in\mathbb{E}$}
        \FOR{$i\in\mathbb{N}_e$}
        \IF{$|r_{e,i}- R^{real}_{e,i}|>\alpha$ %\cwu{is $R^{real}_{e,i}$ defined?}
        }
        \STATE Append ${\bf f}'_{j,1}$ to $\mathbb{L}_{\tau}$.
        \IF{$M^{real}\geq \sum^{|\mathbb{M}|}_{j=1}x_{\tau,\hat{a}_e,e,i,j}{\mathbb{M}}_j$ %\cwu{is $M^{real}$ defined?}
        }
        \STATE $\rho'=\rho_1$, $n^{new}_{e,i}=\lceil \frac{M^{real}}{\sum^{|\mathbb{M}|}_{j=1}x_{\tau,\hat{a}_e,e,i,j}\mathbb{M}_j}\rceil$. %\cwu{is $n^{new}_{e,i}$ defined?}.
        \ELSIF{$\hat{a}_{\tau,e}=3$ and $R^{real}_{e,i}>D^p$}
        \STATE $\rho'=\rho_2$, $n^{new}_{e,i}=\lceil \frac{R^{real}_{e,i}}{D^p}\rceil$.
        \ELSE
        \STATE $\rho'=\rho_3$, $n^{new}_{e,i}=1$.
        \ENDIF
        \STATE ${\bf \epsilon}_{\tau,1:\mu Q}=(1+\rho'\tau){\bf \epsilon}_{\tau,1:\mu Q}$.
        \STATE Replicate %replicas of the
        expert $i$ $n^{new}_{e,i}$ times.
        \ENDIF
        \ENDFOR
        \ENDFOR
        \STATE
        Deploy %$MoE_t$ 
        the MoE model using $(\hat{a}_e, x_{\hat{a}_e,e,i},y_{\hat{a}_e,e,i},\beta)_{\tau}$;
        \STATE $c_{\tau,j}=MoE_{\tau}(input_{j})$. %\cwu{$c_{j,e,i}, Expert_{t,e,i}, input_{e,i}$ are not defined}.
        \ENDFOR
        \STATE
        $c_{\tau}=\frac{1}{J}\sum^J_{j=1}c_{\tau,j}$.
        \STATE $\mathbb{B}_{\tau}\leftarrow\mathbb{B}_{\tau-1}$$\cup(\{{\bf z}_{\tau-1,q}, v_{\tau-1,q}\}_{q\in\{1,\dots,Q\}},c_{\tau})$.
        \STATE ${\bf z}_{\tau,1:\mu Q},v_{\tau,1:\mu Q}\leftarrow {\bf \epsilon}_{\tau,1:\mu Q}-$GS over $\mathbb{B}_{\tau}$, $\mathbb{L}_{\tau}$.% \cwu{GS function is not defined}.
        \STATE ${\bf z}_{\tau,\mu Q+1:Q},v_{\tau,\mu Q+1:Q}\leftarrow {\bf \epsilon}_{\tau,1:\mu Q+1:Q}-$GS over $\mathbb{B}_{\tau}$, $\mathbb{P}$.
        \STATE $\tau=\tau+1$, initialize $\mathbb{L}$.
        \UNTIL{The change of $\min_{\tau\in{1,\dots,\tau}}c_{\tau}$ within $\lambda$ consecutive iterations is below $\zeta$, and record the last iteration index as $\eta$}
        \RETURN$\{\hat{{\bf z}}_{q},\hat{v}_{q}\}_{q\in\{1,\dots,Q\}}=argmin_{\tau\in\{1,\dots,\eta\}}{c_{\tau}}$.
    \end{algorithmic}
\end{algorithm}


%We design a BO algorithm with a multi-dimensional ${\bf e}$-GS to control the entire system. This algorithm controls a feedback processor to fine-tune expert selection prediction, an expert selection predictor, a policy maker, and a serverless computing platform. 

BO is a statistical approach for global optimization of a black-box function, including an objective, variables, a surrogate function to simulate the objective, and an acquisition method to update the variables. BO makes no assumptions about the underlying function format and aims to minimize the number of trials to find a near-optimal solution, reducing tuning costs. 
In our BO algorithm, the black box function corresponds to the billed cost of all MoE layers for MoE inference in a serverless platform. %which depends on the key-value pairs in the dataset table used by the expert predictor.
% \cwu{tell what the black-box function corresponds to in our BO algorithm}. 
Each trial corresponds to one BO iteration which adjusts the key-value table, recomputes expert selection predictions and distributed MoE model deployment. %The tuning costs correspond to the high billed costs resulting from suboptimal MoE deployment due to inaccurate expert selection predictions. \mf{I'm not sure if it is the tuning costs} \cwu{tell what the tuning costs correspond to in our system}. 

The objective of our BO is to minimize the billed cost of all MoE layers. %in the serverless platform. 
The variables are $Q$ key-value pairs in the key-value table $\Omega(\cdot)$ for adjusting expert selection prediction. The surrogate function uses a Gaussian process to simulate the cost of all MoE layers deployed by the policy maker based on expert selection prediction.
For the acquisition method, we design a decaying multi-dimensional ${\bf \epsilon}$-greedy search (GS) to set the variables for the next BO iteration. Traditional %decaying 
single-dimension $\epsilon$-GS, as an acquisition function, decays with each iteration and balances exploration of BO variables and exploitation of high-performing BO variable values  
by selecting the best variable %\cwu{what does best-known variable mean?} 
with probability $1-\epsilon$ and exploring new variable values with probability $\epsilon$ \cite{de2020epsilon}. 
However, as multiple key-value pairs in key-value table need to be adjusted together in a single BO trial, these pairs can be viewed as multi-dimensional variables in our BO, which make %\cwu{why our variables-key/value pairs are multi-dimensional?} in our BO, 
a single-dimension $\epsilon$ insufficient to balance exploration and exploitation in all dimensions. We extend $\epsilon$ to a multi-dimensional vector ${\bf \epsilon}\in\mathbb{R}^Q$. %\cwu{e has been used to denote expert - change the symbol}.

In BO learning, our objective, billed cost of all MoE layers, is obtained on several batches of inference data from an open-source real-world dataset \cite{enwik8,lambda,wmt19} (different datasets can be used for different MoE inference tasks). 
When inaccurate expert selection prediction occurs compared to the ground truth in the profiled data, %by some batches of data in the same MoE task, %\cwu{tell how you know expert selection prediction is inaccurate}, 
we set a limited range of key-value pairs to update as $\mathbb{L}$, where $\mathbb{L}$ includes all positive integers for values and all possible token-to-expert mappings with token IDs limited to those present in these batches of data for keys. %\cwu{what are `training' tokens}, 
 We set a ratio $\mu$, and slow down the decay of the split ${\bf \epsilon}_{1:\mu Q}$ of vector ${\bf \epsilon}$ from the first dimension to the $\mu Q$-th dimension by multiplying ${\bf \epsilon}_{1:\mu Q}$ with a factor greater than 1. %\cwu{explain ${\bf e}_{1:\mu Q}$ and how do you slow down the decay?}. 
The 1st to $\mu Q$-th key-value pairs in our key-value table %variables
are then updated using ${\bf \epsilon}_{1:\mu Q}$ by adjusting the values of keys in $\mathbb{L}$, 
%\cwu{clarify how the key-value pairs are updated within this limited range using ${\bf e}_{1:\mu Q}$}, 
allowing for more exploration on current low-performing key-value pairs. %\cwu{what the inaccurate data is referring to} 
%to improve expert selection prediction accuracy.
Meanwhile, the $\mu Q + 1$-th through the last key-value pairs in the variables are updated by either adjusting the values of keys in $\mathbb{P}$ or by creating new key-value pairs in $\mathbb{P}$ using ${\bf \epsilon}_{\mu Q+1: Q}$. Here, $\mathbb{P}$ is a normal range of key-value pairs to adjust, includeing all positive integers for values, and all possible token-to-expert mappings for keys, where token features can include all possible token IDs assigned by the tokenizer, all possible position IDs, and all possible attention IDs, %(which are the same as token IDs), 
and experts are represented by all possible expert indices.
%\cwu{what is a selection range?} $\mathbb{P}$ (i.e., all token IDs, attention IDs in the tokenizer, position IDs, MOE layer indices, and expert indices) %using ${\bf e}_{\mu Q+1: Q}$. 
This enriches the key-value table by creating new key-value pairs with keys as token-to-expert mappings not present in the profiled data.
%\cwu{tell what are unprofiled data in the table, the 1st to $\mu Q$-th key-value pairs?}.

The BO algorithm with multi-dimensional ${\bf \epsilon}$-GS %to minimize the billed cost of all MoE layers 
is given in Alg.~\ref{alg1}. In the $\tau$-th BO iteration, %\cwu{t has been used a lot to denote different time earlier - change the symbol}, 
${\bf \epsilon}$ decays by being divided by $1+\rho \tau$ with a constant $\rho>0$ (line 3). The dataset table $\Omega_{\tau}$ is updated with key-value pairs $\{{\bf z}_{\tau-1,q}, v_{\tau-1,q}\}_{\forall q \in\{1,\dots,Q\}}$ (line 4). %\cwu{k has been used in top-k so need to change the symbol}, 
where ${\bf z}=\{{\bf f}, e, i\}$. %with ${\bf f}_1$ as token ID, ${\bf f}_2$ as position ID, ${\bf f}_3$ as attention ID, $e\in\mathbb{E}$, and $i\in\mathbb{N}_e$.
Then expert selection is predicted (line 5). The policy maker produces the optimal deployment policy using %three MIQCP solvers and 
the ODS algorithm (lines 6-7).
For the $j$-th batch $input_j$ in BO learning%\cwu{clarify this is batch data in BO instead of real inference serving}
(lines 8-27), at expert $i$ in MoE layer $e$, if predicted counts $r^{e,i}$ and real counts $R^{real}_{e,i}$ of tokens assigned to one replica of this expert
%\cwu{distributions or just concrete selections} 
exceeds a constant $\alpha>0$, token IDs ${\bf f}'_{j,0}$ of the $j$-th batch are recorded for limiting the range of key-value pairs to adjust %\cwu{for what purpose?} 
(line 12) and three cases are discussed (lines 10-21): (i) if the minimal memory $M^{real}$ required by real expert popularity%\cwu{what is the real memory} 
exceeds memory configuration of serverless functions, %\cwu{memory configuration of serverless functions?}, 
$\rho_1<\rho$ is used to decrease the decay rate ${\bf \epsilon}_{\tau, 1:\mu Q}$, and $n^{new}_{e,i}$ is calculated to replicate expert $i$ $n^{new}_{e,i}$ times to satisfy the minimal memory $M^{real}$ %more serverless functions are deployed 
%\cwu{how does decreasing decay rate lead to more serverless functions deployed} 
(lines 13-14, 20-21); (ii) if the size of transferred tokens exceeds the payload size under direct transfer, $\rho_2<\rho_1$ is used to decrease the decay rate ${\bf \epsilon}_{\tau,1:\mu Q}$, and $n^{new}_{e,i}$ is calculated to replicate expert $i$ $n^{new}_{e,i}$ times to ensure that the data size transferred to each replica does not exceed the payload size $D^p$
%\cwu{tell the raionale} 
(lines 15-16, 20-21); (iii) if all constraints in~(\ref{formulation_v1}) are satisfied, %\cwu{in what case - otherwise?} 
$\rho_3<\rho_2$ is used to decrease the decay rate ${\bf \epsilon}_{\tau, 1:\mu Q}$, and we do not replicate expert $i$ to avoid increasing cost %\cwu{why?} 
(lines 17-18, 20-21). Then %the MoE model $MoE_{\tau}$ is deployed (line 25, simulated in general), and 
the billed cost of all MoE layers $c_{\tau,j}$ is computed on the $j$-th batch data $input_j$ on the derived MoE model deployment $MoE_{\tau}$ (lines 25, 26, 28).
%After inference over the requests from real-world dataset,
%\cwu{inference over what requests?}, 
Next the historical set $\mathbb{B}$ in BO to record variables and objectives %\cwu{what is the set of the BO parameters and values?} 
is updated (line 29), and the key-value pairs to adjust is updated by ${\bf \epsilon}$-GS over the historical set %in BO 
and the range of key-value pairs $\mathbb{P}$ and $\mathbb{L} $%\cwu{tell what `new variable is acquired' means in our system} by the %acquisition function 
%e-GS 
(lines 30-31). %The index of BO iteration increases and the limited range of key-value pairs are re-initialized for the next BO iteration (line 32). 
Then BO iterations repeat until the change of the minimal billed cost of all MoE layers within $\lambda$ consecutive iterations is below the threshold $\zeta$ (line 33). %and the optimal key-value pairs to adjust is returned (line 34).
%This BO algorithm runs at the beginning of the MoE model inference on the same batches of tokens to obtain the finetuned expert selection predictor. After finetuning, the model inference continues to work on different new tokens without the BO algorithm.
%\cwu{not clear if the BO algorithm runs throughout the MoE model inference of many batches or just at the beginning of MoE model serving. are the actual model deployments adjusted each time in line 6? i.e., the model deployments keep changing during MoE inference? all these need to be clarified.}

%Therefore, as shown in Fig.~\ref{sysoverview}, the BO processor works as the feedback processor, the expert selection predictor is finetuned by new data patterns, and the policy maker is the MIQCP solver. %This designed BO algorithm aims at minimizing the billed cost of all MoE layers in the inference in serverless computing by iteratively finetuning the expert selection prediction with new data patterns and optimizing the distributed deployment based on the designed all-to-all communication. 

\subsection{Theoretical Analysis} 

%We next analyze the time complexity of Alg.~\ref{alg_optimal_deploy} and Alg.~\ref{alg1}, and the optimality of Alg.~\ref{alg_optimal_deploy} as compared to true optimum of three MIQCP solvers in ($\ref{formulation_v1}$).

\noindent\textbf{Theorem 1.} \textit{Alg.~\ref{alg_optimal_deploy} produces feasible MoE deployment in $O(|\mathbb{E}|)$ time, which achieves a billed cost of all MoE layers upper bounded by a constant ratio of the cost of optimal solutions of (\ref{formulation_v1}).}
%\cwu{why compare Alg.~\ref{alg_optimal_deploy}'s solution to the cost of optimal solutions of the three MIQCP solvers? Alg.~\ref{alg_optimal_deploy}'s solution should be compared to optimal solution of (12)}

\noindent\textbf{Theorem 2.} %\cwu{the Theorem should give time complexity of Alg. 2 till convergence instead of for a preset iteration number T, and also give any optimality of the BO algorithm when converging, expert prediction accuracy?} 
\textit{Alg.~\ref{alg1} converges when the BO iteration index satisfies $\tau>\frac{1+\rho}{\rho-\rho_1}(1-\frac{\delta}{\max_{q\in\{1,\dots,Q\}}\epsilon_{0,q}})$ with an abitrary small positive constant $\delta<\max_{q\in\{1,\dots,Q\}\epsilon_{0,q}}$.
%produces feasible expert selection prediction and MoE deployment %strategies 
%in $O(NJT)$ time, where $T$ is the number of BO iterations, $J$ is the number of training batches, and $N=\sum_{e\in \mathbb{E}}|\mathbb{N}_e|$ is the number of all experts in the MoE model.
}

%\noindent\textbf{Theorem 3. }\textit{The billed cost of all MoE layers achieved by Alg.~\ref{alg_optimal_deploy} is upper bounded by a constant ratio of the cost by optimal solutions of three MIQCP solvers.}
Theorem 1 indicates that the time complexity of Alg.~\ref{alg_optimal_deploy} scales linearly with the number of MoE layers. %as three communication methods provide up to $3|\mathbb{E}|$ solutions of $\hat{a}_e$,$\forall e\in\mathbb{E}$, and selecting $|\mathbb{E}|$ solutions leaves up to $2|\mathbb{E}|$ solutions that can be excluded. %\cwu{briefly give the rationale}. 
Theorem 2 shows that the Alg.~\ref{alg1} converges in a constant bound. %and Theorem 3 indicates that the billed cost from Alg.~\ref{alg_optimal_deploy} is bounded by a constant ratio of the optimal solutions from the MIQCP solvers.
%This ensures the deployment strategies produced are efficient and cost-effective, suitable for large-scale serverless computing environments. 
%These three theorems ensure Alg.~\ref{alg_optimal_deploy} and Alg.~\ref{alg1} can produce efficient and cost-effective deployment strategies for large-scale serverless computing environments. 
% The proof can be found in our technical report and omitted here due to space limit.
% \begin{comment}
The sketch of proods are as follows.
% \cwu{tell where the proofs to the theorems are.}

\noindent\textit{Sketch of Proof 1:} In theorem 1, the time complexity is analyzed in this section. We prove that the billed cost by the optimal solutions \textbf{OPT} of (\ref{formulation_v1}) is lower-bounded by the ideal \textbf{OPT\_LB}. as $\sum_{e\in\mathbb{E}}\min_{a_e\in\mathbb{A}}c_{a_e,e}$.
On the other hand, the billed cost achieved by Alg.~\ref{alg_optimal_deploy} (i.e., \textbf{ALG}) is upper bounded by \textbf{ALG\_UP} as $\sum_{e\in\mathbb{E}}\max_{a_e\in\mathbb{A}}c_{a_e,e}$. 
From Sec~\ref{Deployformulation}, $c_{a_e,e}>\sum_{i\in\mathbb{N}_e}\{T^{h,E}_{e,i}\}+\sum_{i\in\mathbb{N}_e}\{d_{e,i}\}(U_{|\mathbb{M}|}+\min\{1/B_s,1/B_f\})$, and $c_{a_e,e}<\mathbb{M}_{|\mathbb{M}|}G(\sum_{i\in\mathbb{N}_e}\{T^{h,E}_{e,i}\}+\sum_{i\in\mathbb{N}_e}\{d_{e,i}\}(U_{1}+\max\{1/B_s,1/B_f\}+T^{dl})$. Here the known head time $T^{h,E}_{e,i}$ as the first term, the number of tokens multiply the known unit calculation and transfer time as the second term, and $\mathbb{M}_{|\mathbb{M}|}$ and $G$ denotes the known maximal memory size and number of replicas. Then \textbf{ALG}$/$\textbf{OPT}$\leq$\textbf{ALG\_UP}$/$\textbf{OPT\_LB}$\leq$$\mathbb{M}_{|\mathbb{M}|}G(U_{1}+\max\{1/B_s,$$1/B_f\}+T^{dl})$$/(U_{|\mathbb{M}|}+\min\{1/B_s,1/B_f\})$. Proved.

\noindent\textit{Sketch of Proof 2:} In theorem 2, when ${\bf \epsilon}$ decays below an arbitrary small positive constant $\delta<\max_{q\in\{1,\dots,Q\}\epsilon_{0,q}}$, we consider the variables achieving the best objective in BO historical set are always selected by GS. As ${\bf \epsilon}$ decays at the slowest rate $(1+\rho_1\tau)/(1+\rho\tau)$, we set $\max_{q\in\{1,\dots,Q\}\epsilon_{0,q}}(1+\rho_1\tau)/(1+\rho\tau)<\delta$. Proved. 
% \end{comment}


%\jw{add a description on what the theorem indicate and why such a result is important in the proposed setting (e.g., linear scalability with respect to problem size, making it efficient and scalable)}

%\jw{the results seem to be weak, as it becomes looser as problem size increases. Can we obtain a better bound?}

==> Sec5-Evaluation.tex <==
\section{Evaluation}\label{Secevaluation}
\subsection{Experimental Setup}
\noindent\textbf{Testbed.} We run our experiments on AWS Lambda \cite{Amazon}. %Each lambda function is deployed through a Docker image and external storage is on S3 bucket. %AWS Lambda charges users on memory usage and execution time of serverless functions. %\cwu{tell the detailed charging model on AWS Lambda.} 
To build MoE layer images, %for serverless functions,
we use a Dockerfile to define the environment with Python 3.8 and include packages such as \emph{torch} and \emph{transformers}. %which is then used to create and deploy Docker images. 
We implement the BO algorithm with package {\em optuna} \cite{optuna} and MIQCP solvers with package {\em gurobi} \cite{Gurobi}.%\cwu{add citation}. %We form the key-value dataset in expert selection prediction using the data structure {\em Dict}.
%\cwu{tell your implementation of the system on AWS Lambda, e.g., how you build MoE layer images for serverless function, how the BO algorithm and modules are implemented.}
We use two S3 buckets of size 512MB each for external storage. 
We adopt 14 discrete memory size configurations for each serverless function: [128, 768, 960, 1152, 1344, 1536, 1728, 1920, 2112, 2304, 2496, 2688, 2880, 3072] MB. %where 128MB is the minimal memory size of one serverless function. 
We set maximal possible expert replica number as 8.


\vspace{1mm}
\noindent\textbf{MoE Models.} Three common transformer-based dense language models are converted to MoE models with all MLP layers after attention layers converted to MoE layers and a gating network of a linear layer: %calculating the top-$k$ expert indices for each token: %\cwu{tell the nomber of MoE layers in each model, the expert number and the model size}

%\begin{itemize}
    %\item 
$\bullet$ Bert \cite{devlin2018bert}: a 12-layer encoder model with 110 million parameters, converted to 12 MoE layers, with each MoE layer having 4, 8, or 16 experts;

$\bullet$ GPT2 \cite{radford2019language}: a 12-layer decoder model with 1.5 billion parameters, converted to 12 MoE layers, with each MoE layer having 4 experts;

$\bullet$ Bert2Bert \cite{chen2021bert2bert}: a 12-layer encoder-decoder model with 247 million parameters, converted to 24 MoE layers, with each MoE layer having 4 experts.
%\end{itemize}

We run the fill-mask task \cite{fillmask} on Enwik8 \cite{enwik8} and CCnews \cite{ccnews} datasets and the translation task \cite{translation} on the Wmt19 \cite{wmt19} dataset for the BERT model. We conduct the text generation task on the Enwik8 and Lambda \cite{lambda} datasets for the GPT-2 model and on the Enwik8 dataset for Bert2Bert model.

\begin{comment}
\vspace{1mm}
\noindent\textbf{Metrics.} 
We measure expert selection prediction accuracy by calculating the average absolute difference per expert between the real and predicted expert selection numbers \cwu{not clear how difference per expert between the real and predicted expert selection numbers is computed}. %For acquisition functions in the BO algorithm, we assess the impact \cwu{of what on what?} by comparing the expert prediction difference and 
During BO, we assess the expert prediction accuracy of billed cost of all MoE layers. %For overall performance and other comparisons, 
We evaluate performance of BO learned expert prediction and MoE deployment using the billed cost of all MoE layers and the inference throughput.


\vspace{1mm}
\noindent\textbf{Baseline.} 
For expert selection prediction, we use Lina \cite{li2023accelerating} as the baseline. For ODS algorithms, we use random selection and a new MIQCP to combine three MIQCPs using the linearization technique. 
%This technique is described as: $y=y_1$ if $a-b<0$ and $y=y_2$ if $a-b\geq 0$; then $y$ can be linearized as $y=fy_1+(1-f)y_2$, with $-fM\leq a-b\leq (1-f)M$ for a large constant $M$. 
For acquisition functions in the BO algorithm, we use random sampler, single dimension $\epsilon$-GS, and TPE \cite{bergstra2011algorithms} as baselines. For overall performance, we use the following baselines: (1) MoE inference accelerated by the CPU inference optimization method betterTransformer \cite{betterTransformer} on 256 CPUs with 512GB of DRAM powered by two AMD EPYC 7H12 64-Core Processors  (since serverless computing hardly supports GPU), (2) MoE inference without acceleration on the same CPU cluster setup, and (3) MoE inference with LambdaML \cite{lambdaml} as over-provisioning in serverless computing. The over-provisioning baseline applies the maximal memory size for all MoE layers in the memory allocation choices, specifically 3008MB. To our knowledge, this paper is the first to optimize the distributed deployment of MoE model inference in serverless platforms. 
\end{comment}

 \begin{figure}[!t]
 \centering
\includegraphics[width=0.5\textwidth]{evaluation_figs/expert_selection.pdf}
\vspace{-5mm}
 \caption{Average difference per expert between real and predicted expert selection numbers under different MoE models, datasets and tasks.%\cwu{remove `Categories'%; clarify what the different cases in x axis mean}
 }\label{fig_expertselection}
\vspace{-5mm}
\end{figure}

 \begin{figure}[!t]
 \centering
 \subfigure[Bert cost.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/communication_cost_bert.pdf}}
 \subfigure[Bert throughput.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/communication_bert.pdf}}
   \subfigure[GPT2 cost.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/communication_cost_gpt2.pdf}}
 \subfigure[GPT2 throughput.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/communication_gpt2.pdf}}
   \vspace{-3mm}
 \caption{Billed cost and inference throughput of MoE layers with different scatter-gather communication methods %for varying token numbers 
 on AWS Lambda.}\label{fig_comm}
 \vspace{-3mm}
\end{figure}

 \begin{figure}[!t]
 \centering
 \subfigure[Bert.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/ODS_bert.pdf}}
   \subfigure[GPT2.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/ODS_gpt2.pdf}}
   \vspace{-3mm}
 \caption{Billed cost of all MoE layers with different MoE deployment algorithms on AWS Lambda. %\cwu{change `Combined MIQCP' to MIQCP}
 }\label{fig_ODS}
\end{figure}


 \begin{figure}[!t]
 \centering
 \subfigure[Bert cost.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/BO_total_cost_compare_bert.pdf}}
 \subfigure[Bert difference.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/BO_difference_compare_bert.pdf}}
   \subfigure[GPT2 cost.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/BO_total_cost_compare_gpt2.pdf}}
 \subfigure[GPT2 difference.]{
   \includegraphics[width=0.23\textwidth]{evaluation_figs/BO_difference_compare_gpt2.pdf}}
   \vspace{-3mm}
 \caption{Ratio of billed cost and expert prediction difference optimized by BO with different acquisition functions over no BO.%\cwu{extend each figure's width so that the legends do not go outside the plot}
 }\label{fig_BO}
\end{figure}

\begin{figure}[!t]
 \centering
 \subfigure[Bert.]{
   \includegraphics[width=0.5\textwidth]{evaluation_figs/final_result_bert.pdf}}
   \subfigure[GPT2.]{
   \includegraphics[width=0.5\textwidth]{evaluation_figs/final_result_gpt2.pdf}}
   \vspace{-3mm}
 \caption{Billed cost of all MoE layers and inverse of throughput under different expert selection distributions on AWS Lambda and CPU clusters. %\cwu{remove `Categories' from the figures, no need to draw Human reading level speed lines}
 }\label{fig_final_result}
\end{figure}

\subsection{Expert selection prediction} 

We first evaluate accuracy of expert selection prediction learned by our BO framework, by calculating the average absolute difference per expert between the real and predicted counts of tokens assigned to each expert.
%selection numbers\cwu{not clear how difference per expert between the real and predicted expert selection numbers is computed}. 
%We compare with expert selection prediction in Lina \cite{li2023accelerating} as the baseline.
Fig.~\ref{fig_expertselection} shows the %average absolute difference per expert between the real and predicted expert selection numbers 
difference across different MoE models, datasets, and tasks. For a task on a dataset, we use 95$\%$ of this dataset for profiling and evaluate the difference on 10,240 tokens in the dataset. Basic Bert MoE represents the Bert MoE model with 4 experts per MoE layer and top-1 routing for the fill-mask task on Enwiki8. The basic GPT2 MoE and the basic Bert2Bert MoE cases are similar. %denote the cases of GPT2 MoE model and Bert2Bert MoE model with 4 experts and top-1 routing for the generation task on the Enwiki8 dataset. 
Other cases are variations based on these basic setups, e.g, GPT2 Lambda denotes the GPT2 basic setup but changes the dataset to Lambda \cite{lambda} dataset. %\cwu{what is the Lambda dataset?}. 
Across all cases, our method outperforms expert prediction in Lina \cite{li2023accelerating}, as Lina only uses token ID as token feature while our method incorporates token ID, position ID, and attention ID to capture additional information % about profiled tokens
for more accurate profiled probabilities. Compared to top-$1$ routing, the results of top-$2$ routing show that increasing the value of $k$ in top-$k$ gating significantly %reduce the prediction difference,
improves the prediction accuracy, as routing to more experts allows prediction mistakes in one expert to be corrected by the other. When the number of experts increases, the average prediction difference decreases. %because when the total %10,240 
%number of tokens are distributed among more experts, %making 
%the difference appears smaller. %as the number of experts grows.
%Overall, this experiment implies that the benefits of our expert selection prediction method are consistent across different datasets, inference tasks, and model architectures.

\subsection{Scatter-gather communication}
We next evaluate performance of our different scatter-gather communication designs. %We follow the expert parallelism in Sec~\ref{systemoverview} to deploy MoE model on AWS Lambda %\cwu{tell how the model is deployed on AWS Lambda for this all-to-all communication comparison} 
%and vary the number of input tokens. 
We allocate 3008MB of memory to each serverless function and use no expert replicas. 
Fig.~\ref{fig_comm} shows the billed cost of MoE layers and throughput of the entire MoE model %\cwu{throughput of MoE layers only, instead of the entire MoE model?} %on AWS Lambda for varying token numbers 
under different communication methods. %pipelined indirect transfer ($a=1$) with varying scatter degrees $\beta$, non-pipelined indirect transfer ($a=2$), and direct transfer ($a=3$).
The results verify that the optimal scatter-gather communication method varies depending on the number of tokens. %and the desired throughput 
%\cwu{but do you set desired throughput in each case?}. 
For 256 tokens, direct transfer performs best for both Bert MoE and GPT2 MoE. As the number of tokens increases, either pipelined or non-pipelined indirect transfers may perform better, while direct transfer becomes impractical due to payload size limitations; %when no MoE layer replicas distribute the tokens. 
%As the number of tokens grows, 
throughput increases because the time for model downloading and serverless function warm-up is distributed over more tokens. %This indicates that processing larger batches improves inference performance. Overall, the experiment demonstrates that the choice of communication method is scenario-dependent, with no single method consistently dominant over the others across all scenarios.

\subsection{ODS algorithm}
We %follow expert parallelism in Sec~\ref{systemoverview} to 
deploy MoE model for
%\cwu{tell the setup under which this set of experiments are done} 
inference using %a total of 
10,240 tokens on AWS Lambda.
Fig.~\ref{fig_ODS} illustrates the billed cost of all MoE layers using our ODS algorithm, an MIQCP method and a random selection method, under different inference throughput targets. The MIQCP method uses one MIQCP solver to directly solve (\ref{formulation_v1}), and the random method randomly selects the communication method at each MoE layer. %from optimal solutions of solving three MIQCP problems with fixed communication methods. 
We set the target throughput by dividing 10240 tokens by the end-to-end latency limit specified in (\ref{formulation_v1}). %\cwu{but the end-to-end latency limit is for one token, so the throughput should just be 1/end-to-end latency limit}.\mf{in (12), its not for just one token, for all tokens in a batch}
%\cwu{clarify how the combined MIQCP method and a random selection method do the MoE deployment, respectively. Explain how you set desired throughputs in the deployment - note it is the end-to-end latency being set in the optimization.} 
The time limit for searching the optimal solution using the MIQCP approach is set to 180s; for the ODS algorithm with three MIQCP solvers, the search time limit is set to 60s. %\cwu{explain what the runtime means in both algorithm}. 
Our ODS algorithm outperforms other methods. % while the random method delivers the worst results. The combined MIQCP method achieves similar performance as our ODS algorithm at lower desired throughputs. However, 
At higher target throughputs, the MIQCP method fails to derive an optimal solution within 180s. %This is because three MIQCP individually reduce the level of nonlinearity by fixing the communication method $a$, reducing the variables and the problem's complexity. As a result, solutions can be found more quickly under tighter constraints, such as higher throughput.
 % \cwu{explain why complexity high when throughput target is high}.

\subsection{BO algorithm}
For BO learning, we use 10,240 tokens from the Enwiki8 dataset to simulate the inference requests, set $Q=1000$ key-value pairs to update in each BO iteration.%, and run the BO algorithm for least 100 iterations \cwu{shouldn't it stop when bill cost does not change for some iterations?}. 
After BO learning, we test on 100 batches of inference requests from the dataset with batch size of 10240 tokens. Due to the long deployment time on AWS Lambda, we use simulation for this set of evaluation. 

Fig.~\ref{fig_BO} shows the ratio of the billed cost and expert prediction differences optimized by BO with different acquisition functions, to that of no BO, respectively. No BO means that we do not use the BO algorithm to adjust our expert predictor, and the expert selection is predicted by the unadjusted predictor. %\cwu{then what do you do with the expert prediction? just use one batch to compute probabilities?}. %Random method, single $\epsilon$-GS and TPE \cite{bergstra2011algorithms} are samplers in BO. 
The random method randomly adjusts key-value pairs, the single $\epsilon$-greedy sampler uses the same $\epsilon$ for all dimensions of the variables, and the TPE \cite{bergstra2011algorithms} method samples on promising regions of variable range %\cwu{of what} 
based on probabilistic modeling.
% \cwu{explain what the no BO, random, single e-GS, TPE \cite{bergstra2011algorithms} methods do.} 
Our multi-dimension ${\bf \epsilon}$-GS performs best in terms of the billed cost % for all MoE layers 
for both Bert MoE and GPT2 MoE models. %This is because our algorithm individually balances exploration and exploitation for each key-value pair in the dataset table, unlike other methods that apply a uniform approach. 
For BERT MoE, our method achieves the highest expert prediction accuracy. %lowest prediction difference. 
For GPT-2 MoE, our algorithm does not always yield the lowest prediction difference, %and sometimes even the highest.
%This may be 
possibly due to the increase of the number of tokens predicted for the most popular experts: our BO algorithm sets a larger $\epsilon$ for key-value pairs where memory is insufficient due to underestimation of expert popularity, resulting in an overestimation of the most popular experts that are most likely to exceed memory limits.% However, these overestimated predictions do not align with the actual expert selections, leading to reduced prediction accuracy.
% \cwu{why our method increases the number of tokens predicted for the most popular experts and why this leads to lower prediction accuracy}, 
% ensuring they receive adequate memory setup \cwu{why `they receive adequate memory setup' is relevant to low prediction accuracy}.

\subsection{Algorithm overhead}

We dissect the %overhead of the system by considering the 
execution time of the expert selection predictor, the ODS algorithm and the BO algorithm. For expert selection predictor, the time of profiling 100 batches of data is around 28.89 seconds, and the prediction time on 10 batches is around 20.31 seconds. The execution time of the ODS algorithm with three MIQCP solvers is around 2.27s. Our BO algorithm requires around 62.15s per iteration and converges in around 1257.89s. 

\subsection{Overall performance}  
% \cwu{tell this experiment's setup in detail.}
We %follow expert parallelism in Sec~\ref{systemoverview} to 
deploy MoE models on AWS Lambda and a CPU cluster for inference serving of 10,240 tokens. The CPU cluster consists of two 64-core AMD EPYC CPUs with 512GB of DRAM. %\cwu{do you use 256 cores on the two AMD EPYC 7H12 64-Core CPUs? 2X64 does not equal 256}.

Fig.~\ref{fig_final_result} compares the billed cost of all MoE layers and inference throughput of the entire MoE model %\cwu{isn't this the average end-to-end inference time per token? Revise the figures to say inference time per token instead} 
under different expert selection distributions (regarding the count of tokens assigned to each expert), %\cwu{what are the different expert selection distributions?}. 
%The inverse of throughput is set to visually compare throughput with human reading speed \cwu{do you derive this inverse of throughput value (output) or set it as inference time targeting in solving MoE deployment problem (input)? if the former, what is the inference time target set in the experiments?}. 
among: 
(1) {\em Serverless with predicted distribution optimized by BO:} the optimal MoE deployement produced by our BO framework;
%\cwu{explain if this is our design; if so, make it the first case in the figure}.
(2) {\em Serverless with real expert selection distribution:} the optimal MoE deployment produced based on ground truth of expert selections in the MoE inference; %\cwu{what the real distribution means?}. 
(3) {\em Serverless with predicted distribution without BO}: the optimal MoE deployment produced using predicted expert selections %from the expert predictor, which 
that is not adjusted by the BO algorithm;
%\cwu{explain what this case does}. 
 (4) {\em LamdaML \cite{lambdaml}}, which uses the maximum memory allocation for each serverless function on AWS Lambda (3008MB) for inference serving, requires no expert prediction, and uses no replicas for each expert;
 %\cwu{clarify what this design does in terms of MoE inference, expert prediction, MoE model deployment} %as over-provisioning in serverless computing. 
% It applies the maximal memory size for all MoE layers %in the memory allocation choices,
 (5) {\em CPU:} the MoE model is deployed in the CPU cluster, %across available CPUs for inference, 
 with all experts at each MoE layer executing concurrently, requiring no expert prediction;
 % \cwu{tell how MoE inference, expert prediction, MoE model deployment is done in this baseline}. 
 (6) {\em CPU betterTransformer:} MoE deployment in the CPU cluster accelerated by the CPU inference optimization method betterTransformer \cite{betterTransformer}, %which benefits from speedups on CPU 
 through sparsity and fused kernels as Flash Attention. %The MoE deployment is the same as the CPU case.
 % \cwu{tell briefly what betterTransformer does and how expert prediction and model deployment is done in this baseline}. 

For both Bert MoE and GPT2 MoE, our serverless MoE inference design consistently results in lower billed costs, as compared to MoE inference on the CPU cluster. Specifically, serverless MoE inference with predicted expert selection reduces the billed cost by at least 75.67$\%$ compared to CPU cluster-based serving. The throughput in serverless-based MoE serving remains significantly above human reading levels of 3.3 tokens per second. 
The lower throughput in serverless MoE serving compared to CPU cluster-based serving is mainly because non-MoE layer computation is limited to the 3008MB memory size of each serverless function, %\cwu{tell if this is a hard constraint on AWS Lamda?}, 
which is far less than the 512GB available in a common CPU cluster. %This issue can be alleviated by extensive works \cite{yu2021gillis} and \cite{romero2021infaas} on accelerating traditional DNN inference in serverless computing.
%Therefore, comparing serverless throughput to CPU throughput is not fair, and we focus instead on cost. 
Among serverless options, the predicted expert selection distribution optimized by BO outperforms both non-BO methods and over-provisioning with LambdaML. The BO-optimized expert distribution not only reduces the billed cost by at least 43.41$\%$ compared to LambdaML with at most an 18.76$\%$ decrease in throughput, but also closely aligns with the cost of deployment using the real expert distribution.


\iffalse
\begin{table}[!t]
\begin{center}
\caption{Billed cost (unit: $GBs$) of all MoE layers under different setups in serverless computing and in CPU clusters}
\vspace{-3mm}
\begin{tabular}{|c|c|c|}
\hline
&Bert MoE&GPT2 MoE\\\hline
CPU Cluster&$6.06\times10^3$&$7.13\times10^3$\\\hline
Over-Provisioning&$105.87$&$108.57$\\\hline
Random Distribution&$57.53$&$69.54$\\\hline
Predicted Distribution Before Finetuning&$49.86$&$62.69$\\\hline
Predicted Distribution After Finetuning&$48.92$&$61.49$\\\hline
Real Distribution&$42.12$&$57.36$\\\hline

\end{tabular}
\label{final_result}
\end{center}
\vspace{-8mm}
\end{table}

\noindent \textbf{Comparison: } Table~\ref{final_result} shows the billed cost of all MoE layers under different setups in serverless computing and in CPU clusters. Here all-to-all communication design is still adopted  %\cwu{not clear what adopting all-to-all to keep the fairness means} 
under the inference time limit (i.e. 73s for Bert MoE, and 133s for GPT2 MoE in MIQCP) for batch size 64. All setups in serverless computing outperform MoE inference in the CPU cluster. For example, the predicted expert distribution after finetuning reduces the cost by at least 99.14$\%$, as idle resources are still costly in a CPU cluster once rented. Compared to the over-provisioning setup, all setups with MIQCP incur smaller costs, showing the necessity of optimizing deployment. Here the deployment with predicted expert selection distribution after finetuning can reduce the cost by at least 43.36$\%$, approaching the cost of the deployment based on real expert selection distribution. Furthermore, the deployments with predicted expert distributions outperform the deployments with random distributions. %especially the one after finetuning decreasing the cost by at least $11.58\%$.
\fi


==> Sec6-Conclusion.tex <==
\section{Conclusion}
This paper studies optimized MoE model deployment and distributed inference serving on a serverless platform, that effectively predicts expert selection, schedules communication with model execution, and minimizes the overall billed cost of serving MoE models. We propose a Bayesian optimization framework with multi-dimensional $\epsilon$-greedy search to learn expert selections and optimal MoE deployment. %achieving optimal billed cost. 
We design a novel Bayesian decision-making approach for expert selection prediction, %including the token feature design, the posterior calculation, and an adjustable key-value dataset table. We 
propose several scatter-gather communication designs for serverless platforms, % including indirect transfers with flexible pipeline operations via external storage, ordinary indirect transmission, and ordinary direct transmission. We
%formulate optimal deployment of distributed MoE inference on a serverless platform into an MIQCP problem, 
and design an ODS algorithm to decide optimal deployment of distributed MoE inference on a serverless platform. %a billed cost of all MoE layers upper bounded by a constant ratio of the optimal solution.
% proposes an efficient Bayesian optimization framework for billed cost minimization of MoE model inference in a serverless computing platform. The BO framework iteratively finetunes the expert selection prediction and optimizes the distributed MoE model deployment. %based on proposed all-to-all communication designs.
% Our expert selection prediction is based on a Bayesian approach exploiting carefully designed token features. %(i.e. token ID, position ID, and attention ID)  and finetuned the prediction with a new data pattern provided by the BO. 
% We propose efficient all-to-all communication designs tailored to representative serverless computing platforms with flexibly scatter and pipeline operations. %. Given the expert selection prediction results, we 
% We carefully formulate a distributed MoE deployment optimization problem to minimize the billed cost of all MoE layers, and design proven efficient algorithms. %, which can be converted to an MIQCP.
Experiments on AWS lambda validate our designs in reducing the billed cost of all MoE layers by at least 75.67$\%$ compared to CPU clusters while maintaining satisfactory inference throughput.  
As compared to LambdaML in serverless computing,
our designs achieve 43.41$\%$ lower cost with a throughput decrease of at most 18.76$\%$. 
